Automata-based Quantitative Verification

Quantitative analysis of computing systems is an emerging area in automated formal analysis. Such properties address aspects such as costs and rewards, quality measures, resource consumption, distance metrics, etc. Existing solutions for problems in quantitative analysis face two challenges, namely lack of generalizability and separation-of-techniques. Lack of generalizability refers to the issue that solution approaches are specialized to cost model. Different cost models deploy such disparate algorithms that there is no transfer of knowledge from one cost model to another. Separation-of-techniques refers to the inherent dichotomy in solving problems in quantitative analysis. Most algorithms comprise of a structural phase which reasons about the structure of the quantitative system(s) using techniques from automata or graphs, and a numerical phase, which reasons about the quantitative dimension/cost model using numerical methods. The techniques used in both phases are so unlike each other that they are difficult to combine, thereby impacting scalability. This thesis contributes to a novel framework that addresses these challenges. The introduced framework, called comparator automata or comparators in short, builds on automata-theoretic foundations to generalize across a variety of cost models. Comparators enable automata-based methods in the numerical phase, hence eradicating the dependence on numerical methods. In doing so, comparators are able to integrate the structural and numerical phases. On the theoretical front, we demonstrate that these have the advantage of generalizable results, and yield complexity-theoretic improvements over a range of problems in quantitative analysis. On the empirical front, we demonstrate that comparator-based solutions render more efficient, scalable, and robust performance, and are able to integrate quantitative with qualitative objectives.

==> Chapters/Comparator/Abstract.tex <==
The notion of comparison between system runs is fundamental in formal verification.  This concept is implicitly present in the verification of qualitative systems, and is more pronounced in the verification of quantitative systems.  In this work, we identify a novel mode of comparison in quantitative systems: the online comparison of the aggregate values of two sequences of quantitative weights. This notion is embodied by {\em comparator automata} ({\em comparators}, in short), a new class of automata that read two infinite sequences of weights synchronously and relate their aggregate values.

We show that {aggregate functions} that can be represented with B\"uchi automaton result in
comparators that are finite-state and accept by the B\"uchi condition as well. Such {\em $\omega$-regular comparators} further lead to generic algorithms for a number of well-studied problems, including the quantitative inclusion and winning strategies in quantitative graph games with incomplete information, as well as related non-decision problems, such as obtaining a finite representation of all counterexamples in the quantitative inclusion problem.

We study comparators for two aggregate functions: discounted-sum and limit-average.  We prove that the discounted-sum comparator is $\omega$-regular iff the discount-factor is an integer.  
Not every aggregate function, however, has an $\omega$-regular comparator. Specifically, we show that the language of sequence-pairs for which limit-average aggregates exist is neither $\omega$-regular nor $\omega$-context-free.  Given this result, we introduce the notion of {\em prefix-average} as a relaxation of limit-average aggregation, and show that it admits $\omega$-context-free comparators.


==> Chapters/Comparator/Application.tex <==
In this section we apply the discounted-sum comparator to solve some open problems, namely the discounted-sum quantiataive inclusion problem (Section~\ref{Sec:Inclusion}) and games with imperfect information under discounted-sum aggregate function (Section~\ref{Sec:ImperfectInfo}).  






==> Chapters/Comparator/DSComparator.tex <==
The discounted-sum of an infinite sequence $A$ with a rational discount factor $d = \frac{p}{q}>1$, denoted by $\DSum{A}{d}$, is defined as $\Sigma_{i=0}^{\infty} A[i] / d^{i}$. 
The discounted-sum aggregate function is used to model the weight (or reward) of various systems, mostly in economics and systems with discounted futures. 
%This section deals with the discounted-sum comparator, the insights behind its construction~\ref{Sec:DiscountedSum}, and its applications~\ref{Sec:App}.


%\subsection{Discounted sum comparator}
$\label{Sec:DiscountedSum}
$\input{Section/DS}



==> Chapters/Comparator/Prelims.tex <==
\section{Aggregate functions}
\label{Sec:AggregateFunctionDef}

\subsubsection*{Discounted-sum aggregate function}


Discounted-sum (DS) is a commonly appearing mode of aggregation which captures the intuition that weights incurred in the near future are more significant than those incurred later on~\cite{AHR2003}. The {\em discount-factor} is a rational-valued paramater that governs the rate at which weights loose their significance in the DS. 


Let $A = A[0]A[1]\dots$ be an infinite weight sequence. Let $A[i]$ denote the i-th element of the sequence, for all $i\geq 0$.  Let $d >1$ be the rational-valued discount-factor. Then the discounted-sum of $A$ w.r.t. discount-factor $d$, denoted by $\DSum{A}{d}$, is defined as 
\begin{align}
	\DSum{A}{d} &= \sum_{i=0}^{|A|-1} \frac{A[i]}{d^{i}}
\end{align}


DS is a preferred mode of aggregation across several domains including
reinforcement learning~\cite{sutton1998introduction}, planning under uncertainty~\cite{puterman1990markov}, and game-theory~\cite{osborne1994course}. One reason behind its popularity is that DS is known to exist for all bounded infinite-length weight sequences, since its value is guaranteed to converge.
Yet another property of mathematical as well as utilitarian interest is that DS over infinite and finite sequences can approximate the limit-average and sum aggregation functions, respectively, as shown in Section~\ref{Sec:AggregateFunction}.



The central result of this section is that whether DS aggregation function is $\omega$-regular or not,  is dependent solely on the discount-factor.


\subsubsection*{Limit-average aggregate function}



The limit-average of an infinite sequence $M$ is the point of convergence of the average of prefixes of $M$,. 
Let $\Sum{M[0,n-1]}$ denote the sum of the $n$-length prefix of sequence $M$.
The {\em limit-average infimum}, denoted by $\LAInf{M}$, is defined as $\liminf{n}{\infty}{\frac{1}{n}\cdot \Sum{M[0,n-1]}}$. Similarly, the {\em limit-average supremum}, denoted by $\LASup{M}$, is defined as $\limsup{n}{\infty}{\frac{1}{n}\cdot \Sum{M[0,n-1]}}$. 
The limit-average of sequence $M$, denoted by $\LA{M}$, is defined {\em only if} the limit-average infimum and limit-average supremum coincide, and then $\LA{M} = \LAInf{M}$ ($=\LASup{M}$).  Note that while limit-average infimum and supremum exist for all bounded sequences, the limit-average may not. 
To work around this limitation of limit-average, most applications simply use limit-average infimum or limit-average supremum of sequences~\cite{brim2011faster,chatterjee2010quantitative,chatterjee2005mean,zwick1996complexity}. 
However, the usage of limit-average infimum or limit-average supremum in liu of limit-average for purpose of comparison can be misleading. 
For example, consider sequence $A$ s.t. $\LASup{A} = 2$ and $\LAInf{A} = 0$, and sequence $B$ s.t. $\LA{B} = 1$. Clearly,  limit-average of $A$ does not exist. So while it is true that$ \LAInf{A} < \LAInf{B}$, indicating that at infinitely many indices the average of prefixes of $A$ is lower, this renders an incomplete picture since at infinitely many indices, the average of prefixes of $B$ is greater as $\LASup{A} = 2 $.


\subsubsection*{$\omega$-regular aggregate function}
 
 Given an integer base $\beta\geq 2$, its {\em digit set} is $\mathsf{Digit}(\beta) =\{0,\dots, \beta-1\}$. Let $x \in \Re$, then there exist unique words $\mathsf{Int}(x, \beta) = z_0z_1\dots \in \mathsf{Digit}(\beta)^*\cdot 0^\omega $ and $\mathsf{Frac}(x, \beta)=f_0f_1\dots \notin \mathsf{Digit}(\beta)^*\cdot (\beta-1)^\omega$ such that $|x| = \Sigma_{i=0}^\infty \beta^i \cdot z_i + \Sigma_{i=0}^\infty \frac{f_i}{\beta^i}$.  
 Thus, $z_i$ and $f_i$ are respectively the $i$-th
 least significant digit in the base $\beta$ representation of the
 integer part of $x$, and the $i$-th most significant digit in
 the base $\beta$ representation of the fractional part of $x$.
 Then, a real-number $x \in \Re$ in base $\beta$ is represented by $\mathsf{rep}(x, \beta) = \mathsf{sign} \cdot  (\mathsf{Int}(x, \beta),\mathsf{Frac}(x, \beta) )$, where $\mathsf{sign} = +$ if $x \geq 0$, $\mathsf{sign} = -$ if $x<0$, and $(\mathsf{Int}(x, \beta),\mathsf{Frac}(x, \beta) )$ is the interleaved word of $\mathsf{Int}(x, \beta)$ and $\mathsf{Frac}(x, \beta)$.
 Clearly, $x = \mathsf{sign}\cdot |x| = \mathsf{sign}\cdot (\Sigma_{i=0}^\infty \beta^i \cdot z_i + \Sigma_{i=0}^\infty \frac{f_i}{\beta^i})$.
 For all integer $\beta\geq 2$, we denote the alphabet of representation of real-numbers in base $\beta$ by $\mathsf{AlphaRep}(\beta)$.
 We adopt the definitions of function automata and regular functions~\cite{chaudhuri2013regular} w.r.t. aggregate functions as follows:
 \begin{Def}[Aggregate function automaton, $\omega$-Regular aggregate function]
 	\label{def:aggregateregular}
 	Let $\Sigma$ be a finite set, and $\beta\geq 2$ be an integer-valued base. 
 	A B\"uchi automaton $\A$ over alphabet $\Sigma\times\mathsf{AlphaRep}(\beta)$ is an {\em aggregate function automata of type $\Sigma^\omega\rightarrow\Re$} if the following conditions hold:
 	\begin{itemize}
 		\item For all $A \in \Sigma^\omega$, there exists at most one $x \in \Re$ such that $(A,\mathsf{rep}(x,\beta)) \in \L(\A)$, and
 		
 		\item For all $A \in \Sigma^\omega$, there exists an  $x \in \Re$ such that $(A,\mathsf{rep}(x,\beta)) \in \L(\A)$
 	\end{itemize}
 \end{Def}
 
 
 $\Sigma$ and $\mathsf{AlphaRep}(\beta)$ are the {\em input} and {\em output} alphabets, respectively. An aggregate function $f:\Sigma^\omega\rightarrow \Re$ is {\em $\omega$-regular} under integer base $\beta \geq 2$ if there exists an aggregate function automaton $\A$ over alphabet $\Sigma\times\mathsf{AlphaRep}(\beta)$ such that for all sequences $A \in \Sigma^\omega$ and  $x\in \Re$, $f(A) = x$ iff $(A,\mathsf{rep}(x,\beta)) \in L(\A)$.
 
 
 
  

==> Chapters/Comparator/RelatedWork.tex <==
%\noindent
%{\it Related Work}
The notion of comparison has been widely studied in quantitative settings. Here we mention only a few of them. Such aggregate-function based notions appear in weighted automata~\cite{AlmagorBokerKupferman,droste2009handbook}, quantitative games including mean-payoff and energy games~\cite{degorre2010energy}, discounted-payoff games~\cite{andersen2013fast,andersson2006improved}, in systems regulating cost, memory consumption, power consumption, verification of quantitative temporal properties~\cite{de2004model,de2004linear},  and others. Common solution approaches include graph algorithms such as weight of cycles or presence of cycle~\cite{karp1978characterization}, linear-programming-based approaches,  fixed-point-based approaches~\cite{chatterjee2010energy}, and the like. 
The choice of approach for a problem typically depends on the underlying aggregate function. In contrast, in this work we present an automata-theoretic approach that unifies solution approaches to problems on  different aggregate functions. We identify a class of aggregate functions, ones that have an $\omega$-regular comparator, and present generic algorithms for some of these problems. 



While work on finite-representations of counterexamples and witnesses in the qualitative setting is known~\cite{baier2008principles}, we are not aware of such work in the quantitative verification domain. 
This work can be interpreted as automata-theoretic  arithmetic, which has been explored in regular real analysis~\cite{chaudhuri2013regular}. 



==> Chapters/Comparator/regular.tex <==
\section{$\omega$-Regular aggregate functions}
\label{Sec:RegularAggFunctions}

$\omega$-regular aggregate functions were introduced by Chaudhuri et. al. in their seminal work on relating arithmetical operations to $\omega$-regular automata~\cite{chaudhuri2013regular}}. 
This chapter explores the connections between {\em $\omega$-regular aggregate functions} and $\omega$-regular comparators in an attempt at establishing a formal criteria to for which aggregate function permit $\omega$-regular comparators. Our investigate has resulted in a one-sided connection between the two.
We discover that $\omega$-regular aggregate functions entail $\omega$-regular comparators. However, we are unable to prove the other direction. 
Hence it is still  unknown whether the existence of an $\omega$-regular comparator for an aggregate function $f$ implies that function $f$ is also $\omega$-regular?. 
From examples, we know that discounted-sum with integer discount factor and limsup/liminf are $\omega$-regular. Therefore, at this point we describe this direction as a conjecture, and hope that it will be proven formally  later on.

We begin with defining $\omega$-regular functions. 
 


==> Chapters/anytime/Abstract.tex <==
\begin{abstract}

{\em Discounted-sum inclusion} (DS inclusion, in short) formalizes the goal of comparing quantitative dimensions of systems such as cost, resource consumption, and the like, when the mode of aggregation for the quantitative dimension is discounted-sum aggregation. While DS inclusion is \cct{PSPACE}-complete for integer discount factors, its decidability is still unknown for non-integer discount factors. 
To this end, this work presents an {\em anytime algorithm} for DS inclusion with non-integer discount factor $1<d<2$ on finite sequences. The anytime algorithm either terminates and returns whether DS inclusion holds or not, or it quickly generates an approximation of DS inclusion and proceeds to generate progressively tighter approximations over time. Furthermore, our anytime algorithm is guaranteed to terminate if DS inclusion does not hold on an input instance. 
In doing so, our work presents the first pragmatic solution for DS inclusion with non-integer discount factors.


\end{abstract}



==> Chapters/anytime/Section/related.tex <==
\section{Related work and future directions}

Two contrasting approaches have been developed for DS inclusion so far, namely (a). comparator-based automata-theoretic approach~\cite{BCVFoSSaCS18,BCVCAV18,BVCAV19}, and (b). DS-automata determinization followed by linear programming~\cite{boker2014exact,chatterjee2010quantitative}.  
These approaches work when the discount factor is an integer but neither extends to non-integer discount factors~\cite{BCVlmcs2019,boker2014exact}.
This work tackles DS inclusion for non-integer discount factors. The natural choice for this is to explore approximation methods.  
But, as shown in this work, the decidability of approximation of DS inclusion is also unknown. 

As a consequence, we turn to anytime algorithms to solve DS inclusion. 
In this work, we use comparator-based approaches to design the  algorithm. We construct comparators for aggregate functions that represent approximations of discounted-sum, and use those to design the critical sub-procedures of the anytime algorithm. 
It remains to be seen whether techniques based on {\em approximations} of DS determinization, as shown in~\cite{boker2014exact}, followed by linear programming leads to a co-recursively enumerable anytime algorithm for DS inclusion.
%can be utilized to develop an anytime algorithm. 
We suspect that even there one would have to develop separate partial solutions for the over- and under-approximations of DS inclusion, and wrap them up in a recursive procedure, just as we have exhibited in this work.

One reason for not exploring an anytime algorithm using approximation of DS determinization in this work is rooted in practical scalability. 
Recent empirical comparison of comparator-based vs. DS determinization-based approaches for DS inclusion with integer discount factors have shown that the former comprehensively outperforms the later in practice because DS determinization is excessively prohibitive~\cite{BCVCAV18,BVCAV19}.
Since approximate DS determinization relies on techniques similar to DS determinization, one would expect approximation of DS determinization to be prohibitive as well. 
Having said that, the jury is still open on which is more scalable: our comparator-automata based anytime algorithm or approximate DS determinization approach (if it exists). An empirical evaluation may lead to algorithmic optimizations and render valuable insights into the internal workings of the antyime algorithm(s).

%Having said that, only an empirical evaluation between comparator-based anytime algorithm and approximate DS determinization-based anytime algorithm (if it exists) can render a concrete reason. We leave these two questions (a) whether an approximate DS determinization-based anytime algorithm exists, (b) If so,  an empirical evaluation to future investigations. 


Finally, the decidability of DS inclusion for non-integer discount factors is still open. 
Various independent results indicate, but do not prove, that it may be  undecidable.
These results include  non-determinizability of DS automata with non-integer discount factor, non-regularity of DS comparator with non-integer discount factor, target discounted-sum~\cite{boker2015target},  non-regularity of discounted-sum with non-integer bases~\cite{akiyama2005representation}, undecidability of quantitative inclusion with sum aggregation~\cite{AlmagorBokerKupferman}, and so on. Despite these many attempts,  decidability of DS inclusion continues to be an open problem. 

%Prior indication of the undeci

%Earlier work on anytime algorithms use them in a myriad of applications in artificial intelligence to combat computational complexity or practical infeasibility~\cite{horsch1998anytime,horvitz2013bounded,lawler1985traveling,wallace1996anytime,zilberstein1996using}.
%Prior work employ anytime algorithms in various applications in artificial intelligence~\cite{zilberstein1996using} including navigation~\cite{lawler1985traveling}, decision-making under uncertainty~\cite{horsch1998anytime}, constraint satisfaction~\cite{wallace1996anytime}, probabilistic inference~\cite{horvitz2013bounded}. Despite prevalence in AI, anytime algorithms are under-explored in formal methods with few  appearances in anytime verification and quantitative abstraction refinement~\cite{cerny2013quantitative}.

==> Chapters/anytime/Section/upper.tex <==


This section describes  Algorithm $\upperInc$ - the second sub-procedures in  our anytime algorithm for DS inclusion. 
Given inputs DS automata $P$ and $Q$, discount factor $1<d<2$ and approximation factor $0<\varepsilon<1$, $\upperInc$ $(P,Q,d,\varepsilon)$ either returns $P \subseteq Q$ holds or  $P\subseteq Q - d\cdot\varepsilon$ does not hold.
As earlier, these outcomes are not {\em mutually exclusive}. In these cases, the algorithm may return either of the outcomes as they are both sound. 

The design of $\upperInc$ follows that of $\lowerInc$ very closely. 
Intuitively, $\upperInc$ solves whether $P$ is $f$-included in $Q$ where aggregate function $f$ is the upper approximation of discounted-sum. Hence, it follows the same three stages:
Define the upper approximation of discounted-sum (\textsection~\ref{Sec:upperApprox}), construct its regular comparator (\textsection~\ref{Sec:lowerComparator}), use the regular comparator to design $\upperInc$ (\textsection~\ref{Sec:lowerIncAlgo}).
For sake of completeness, we state and prove all major results.

\subsection*{Section~\ref{Sec:upperInc}.1. Upper approximation of discounted-sum}
\label{Sec:upperApprox}

In the first stage we define the upper approximation of discounted-sum so that its recoverable gap obeys the bounded non-zero minimal difference property. 
%This section defines upper approximation of discounted sum  when $1<d<2$ so that its comparator is regular. 


For a rational number $x \in \mathbb{Q}$, let $\roundU{x}$ denote the smallest integer multiple of resolution that is more than or equal to $x$. 
Formally, $\roundU{x} = i\cdot 2^{-(p+k)}$ for an integer $i \in \Z$  such that for all $j\in \Z$,  $j\cdot 2^{-(p+k)} \geq x$ implies  $i\leq j$. 
The upper gap value and upper approximation of discounted sum are defined as follows:


\begin{lemma}
\label{lem:UpperRound}
Let $k,p >0$ be rational-valued parameters. Then,
for all real values $x\in \Re$, $0\leq  \roundU{x} -x < 2^{-(p+k)}$.
\end{lemma}
\begin{proof}
There exists a unique  integer $i \in \Z$ and $0\leq b  < 2^{-(p+k)}$ such that $x = i\cdot 2^{-(p+k)} - b$. Then, $ \roundU{x} = i\cdot 2^{-(p+k)}$. Therefore, we get that $0\leq \roundU{x} - x < 2^{-(p+k)}$.
\qed
\end{proof}

\begin{lemma}[Monotonicity]
\label{lem:uppermono}
Let $k,p >0$ be rational-valued parameters. Then,
if $x\geq y$, then $\roundL{x} \geq \roundL{y}$. 
\end{lemma}
\begin{proof}
The proof of this is very similar to that of Lemma~\ref{Lem:LowerMono}.
\qed
\end{proof}


\begin{definition}[Upper gap]
\label{def:approxDSUpper}
Let $W$ be a finite weight sequence. The {\em upper  gap} of $W$ with discount factor $d = 1+2^{-k}$ and approximation factor $\varepsilon=2^{-p}$, denoted $\gapU{W}$, is 
\[
\gapU{W} = 
\begin{cases}	
0, \text{ for } |W| = 0 \\
\roundU{\gapU{U}+u} \text{ for } W = U\cdot u
\end{cases}
\]
\end{definition}





\begin{definition}[Upper approximation of discounted-sum]
\label{def:approxDSUpper}
Let $W$ be a finite weight sequence.
The {\em upper approximation of discounted sum}, called upper DS, for weight sequence $W$ with discount  factor $d = 1+2^{-k}$ and approximation factor $\varepsilon=2^{-p}$ is denoted by and defined as 
$$\DSumU{W} = \gapU{W}/d^{|W|-1}$$
\end{definition}

Definition~\ref{def:approxDSUpper} is completed by showing the it indeed corresponds to an upper approximation of discounted sum. This requires a basic lemma statement:

\begin{lemma}
\label{lem:UpperGapDifBounded}
Let $k,p>0$ be rational-valued parameters. Let $d = 1+2^{-k}$ be the non-integer, rational discount factor and $\varepsilon=2^{-p}$ be the approximation  factor. Let $W$ be a finite non-empty weight sequence.
 Then $0\leq \gapU{W} - \gap{W} < \gap{R_{|W|}}$.
\end{lemma}
\begin{proof}
The proof argument follows by induction on length of weight sequence $W$. It makes use of Lemma~\ref{lem:UpperRound} and Lemma~\ref{lem:uppermono}, and closely follows the proof presented in 
Lemma~\ref{lem:LowerGapDifBounded}.
\qed
\end{proof}



\begin{theorem}
\label{thrm:ApproxDSUpper}
Let $d = 1+2^{-k}$ be the  discount factor and $\varepsilon=2^{-p}$ be the approximation  factor, for rationals $p,k>0$. 
Then for all weight sequences $W$, 
 $0\leq \DSumU{W} - \DSum{W}{d} < d\cdot \varepsilon$.
\end{theorem} 

\begin{proof}
The proof argument makes use of Lemma~\ref{lem:UpperGapDifBounded} and closely follows that of Theorem~\ref{thrm:ApproxDSLower}.
\qed
\end{proof}

\subsection*{Section~\ref{Sec:upperInc}.2. Comparator automata for upper approximation of DS}
\label{Sec:UpperComparator}

This section constructs a regular comparator for the upper DS defined above. The construction here differs from that of the comparator for lower DS in only one aspect - the values of the thresholds within which it is sufficient to track the value of upper gap in. In this section, we define the comparison language and its comparator automata, prove the necessary thresholds and give the complete construction of the comparator.

\begin{definition}[Comparison language for upper approximation of DS]
\label{def:comparisonAutUpper}
Let $\mu>0$ be an integer bound, and $k,p$ be positive rationals.
The {\em comparison language for upper approximation of discounted sum} with discount factor $d = 1+2^{-k}$, approximation factor $\varepsilon=2^{-p}$, upper bound $\mu$ and inequality relation $\mathsf{R} \in \{\leq, \geq \}$ is a language 
that accepts 
bounded and finite weight sequence $W  \in \Sigma^*$ iff $\DSumU{W}$ $\mathsf{R}$ $0$ holds. 
\end{definition}

\begin{definition}[Comparator automata for upper approximation of DS]
\label{def:comparatorAutUpper}
Let $\mu>0$ be an integer bound, and $k,p$ be positive rationals.
The {\em comparator automata for upper approximation of discounted sum} with  discount factor $d = 1+2^{-k}$, approximation factor $\varepsilon=2^{-p}$, upper bound $\mu$ and inequality relation $\mathsf{R} \in \{\leq, \geq \}$ is an automaton that accepts 
the corresponding comparison language. 
\end{definition}

We establish the range of sufficient values for the upper gap. The new bounds are as follows:

\begin{lemma}
\label{lem:compartorUpperThresholds}
Let $\mu>0$ be an integer bound. 
Let $k,p$ be positive rationals  s.t. $d = 1+2^{-k}$ is the discount factor, and $\varepsilon=2^{-p}$ is the approximation factor.
Let $W$ be a finite and bounded weight sequence. 

\begin{enumerate}
    \item If $\gapU{W}\leq -\mu \cdot 2^{k} - 2^{-p}$ then for all $u \in \{-\mu, \dots, \mu\}$, $\gapU{W\cdot u}\leq -\mu \cdot 2^{k} - 2^{-p}$.
    \item If $\gapU{W} \geq \mu \cdot 2^{k}$, then for all $u \in \{-\mu, \dots, \mu\}$, $\gapU{W\cdot u} \geq \mu \cdot 2^{k}$.
\end{enumerate}
\end{lemma}

\begin{proof}
Part 1. 
Let $W$ and $u$ be as defined above. 
Then 
$\gapU{W\cdot u} = \roundU{d\cdot \gapU{W} +  u}$. From Lemma~\ref{lem:UpperRound}, we get that
$\gapU{W\cdot u} \leq d \cdot \gapU{W}+ u + 2^{-(p+k)}$.
From our assumption, we further get that $\gapU{W\cdot u} \leq d \cdot -(\mu\cdot 2^{k}+2^{-p} )+ u  = (1+ 2^{-k}) \cdot-(\mu\cdot 2^{k} + 2^{-p}) + u +2^{-(p+k)}= -\mu\cdot 2^{k} - \mu - 2^{-p} - 2^{-(p+k)} + u + 2^{-(p+k)} \leq -(\mu\cdot 2^k + 2^{-p})$.

Part 2. 
Let $W$ and $u$ be as defined above. 
Then 
$\gapU{W\cdot u} = \roundU{d\cdot \gapU{W} + u}$. From Lemma~\ref{lem:UpperRound}, we get that $\gapU{W\cdot u} \geq  d \cdot \gapU{W}+ u $. Further, from our assumptions we get that $\gapU{W\cdot u} \geq  d \cdot \mu \cdot 2^{k}+ u
= (1+2^{-k}) \cdot \mu \cdot 2^{k} + u  =
\mu\cdot 2^k+  \mu +  u  \geq \mu\cdot 2^k$, since $\mu \geq u$. 

\qed
\end{proof}

\subsubsection{Construction}
%\textbf{\textsf{Construction}}

Let $\mu>0$,  $d = 1+2^{-k}$, $\varepsilon=2^{-p}$  be the upper bound, discount factor and approximation factor, respectively.
Let $\thresh_l$ be the largest integer such that $\thresh_l\cdot 2^{-(p+k)} \leq -\mu \cdot 2^{k}$. Let $\thresh_u$ be the smallest integer such that
$\thresh_u \cdot 2^{-(p+k)} \geq \mu\cdot 2^{k} + 2^{-p}$.
Note, the thresholds are from Lemma~\ref{lem:compartorUpperThresholds}.
For relation $\mathsf{R} \in \{\leq, \geq\}$,
construct DFA $\compU(\mu,k,p,\mathsf{R}) = (\State, \Start, \Sigma, \delta, \Final)$ as follows:


\begin{itemize}
	\item $\State = \{\thresh_l, \thresh_l+1,\dots, \thresh_u \}$,
	 $\Start = \{0\}$ and 
	 $\Final = \{i | i\in S \text{ and $i$ $R$ $0$}\}$
	
	\item Alphabet $\Sigma = \{-\mu, -\mu+1,\dots, \mu-1, \mu\}$
	\item Transition function $\delta\subseteq \State \times \Sigma \rightarrow \State$ where $(s,a,t) \in \delta$ then:
	\begin{enumerate}
		\item \label{Trans:SelfLoop} If $s = \thresh_l$ or $s= \thresh_u$, then $t = s$ for all $a \in \Sigma$
		\item Else, let $\roundU{d\cdot s \cdot 2^{-(p+k)} + a} = i \cdot 2^{-(p+k)}$ for an integer $i$
		\begin{enumerate}
			\item \label{Trans:IntState} If $\thresh_l \leq i \leq \thresh_u$, then $t = i$
			
			\item \label{Trans:leq} If $i> {\thresh_h}$, then $t = \thresh_u$
			\item \label{Trans:geq} If $i< {\thresh_l}$, then $t = \thresh_l$
		\end{enumerate}
		
	\end{enumerate}
\end{itemize}
\label{thrm:Comparatorupper}

\begin{theorem}
\label{thrm:Comparatorupper}
Let $\mu>0$ be and integer upper bound. Let $k,p>0$ be rational parameters s.t. $d = 1+2^{-k}$ is the  discount factor and $\varepsilon=2^{-p}$ is the approximation parameter. 
 DFA $\compU(\mu,k,p,\mathsf{R}) $ accepts a finite weight sequence $W \in \Sigma^*$ iff $\DSumU{W}$ $\mathsf{R} $ $ 0$.
 DFA $\compU(\mu,k,p,\mathsf{R}) $ has $\O(\mu\cdot 2^{2k+p})$ states.
\end{theorem}


\input{Section/far.tex}

==> Chapters/anytime/macro.tex <==
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{hyperref}
%\usepackage[bookmarks=false]{hyperref}
\usepackage{listings}
\usepackage{makeidx}  % allows for indexgeneration
\usepackage{smallsec} % self-style file
%\usepackage[compact]{titlesec}
\usepackage{subcaption}
\usepackage{url}
\usepackage{wrapfig}

%tikz package 
\usepackage[graphicx]{realboxes}
\usepackage{tikz}
\tikzset{elliptic state/.style={draw,ellipse}}
\usetikzlibrary{shapes,shapes.geometric,arrows,fit,calc,positioning,automata,}
\usetikzlibrary{automata,positioning}
\usepackage{tikz-qtree}
\usepackage{float}
\usepackage{floatflt}

%General macros
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\Z}{\mathbb{Z}}
\renewcommand*{\L}{\mathcal{L}}
\renewcommand*{\O}{\mathcal{O}}
\newcommand{\ol}[1]{\overline{#1}}
\renewcommand*{\Re}{\mathbb{R}}
\newcommand*{\cct}[1]{\textsf{#1}}

%Approximate inclusion algorithm
\newcommand*{\approxInc}{\mathsf{anytimeInclusion}}
\newcommand*{\rationalInc}{\mathsf{DSInclusion}}

%General math macros
\renewcommand*{\mod}[1]{|#1|}
\newcommand*{\ceil}[1]{\lceil #1 \rceil}
\newcommand*{\floor}[1]{\lfloor #1 \rfloor}

%General automata-theroetic notations
\newcommand*{\A}{\mathcal{A}}
\newcommand*{\Statess}{\mathit{S}}
\newcommand*{\State}{S}
\newcommand*{\Start}{s_I}
\newcommand*{\Final}{\mathcal{F}}
\newcommand*{\StartState}{{\mathit{Init}}}
\newcommand*{\AcceptingStates}{S_{acc}}
\newcommand*{\wt}{\mathit{wt}}
\newcommand{\compL}{\mathsf{compLow}}
\newcommand{\compU}{\mathsf{compUpper}}

%macros for DS
\newcommand*{\DSum}[2]{\mathit{DS}({#1}, {#2})}
\newcommand*{\MaxC}{\mathit{maxC}}
\newcommand{\thresh}{\mathsf{T}}
\newcommand{\roundL}[1]{\mathsf{roundLow}(#1,k,p)}
\newcommand{\roundU}[1]{\mathsf{roundUpper}(#1,k,p)}
\newcommand{\gap}[1]{\mathsf{gap}(#1,d)}
\newcommand{\gapL}[1]{\mathsf{gapLower}(#1,k,p)}
\newcommand{\gapU}[1]{\mathsf{gapUpper}(#1,k,p)}
\newcommand{\DSumL}[1]{\mathsf{DSLow}(#1,k,p)}
\newcommand{\DSumU}[1]{\mathsf{DSUpper}(#1,k,p)}

\newcommand{\todo}[1]{\textbf{TODO}{#1}}

%Inclusion algo macros
\newcommand{\lowerInc}{\mathsf{lowApproxDSInc}}
\newcommand{\upperInc}{\mathsf{upperApproxDSInc}}
\newcommand{\AugmentWtAndLabel}{\mathsf{augmentWtAndLabel}}
\newcommand{\MakeDifProduct}{\mathsf{productDif}}
\newcommand{\dominatedWitness}{\mathsf{dominatedWitness}}
\newcommand{\dominated}{\mathsf{dominated}}


\frenchspacing

==> Chapters/approximatesynthesis.tex <==
\chapter{A case study on synthesis with quantiative constraints}
\label{ch:approximationsyn}

Separation-of-techniques becomes prominent in synthesis with quantitative and qualitative constraints. The cause it is that 
qualitative constraint are solved via reduction to games with $\omega$-regular objectives while quantitative constraints are have so far been solved via optimization techniques. As a result, existing work on synthesis of qualitative and quantitative constraints can ensure one of the two: They either offer rich expressiveness in qualitative and quantitative constraints, or offer strong guarantees on the satisfaction of the constraints.  In this chapter, we will investigate comparator automata to  combine qualitative and quantitative constraints in a way that does not compromise on expressiveness and theoretical guarantees.

\section{Introduction}



\section{Motivating example}

Write about social distancing example. 

Consider a robot (Player $P_1$) in a grid world.
Suppose there is a human in the grid, say $P_0$. 
Suppose the human and robot take turns in moving around the grid. The robot has to expend its battery to make each movement. The grid also has two charging stations, where the robot may recharge its battery.

Our objective is to design a strategy for robot $P_1$ so that it can roam around the grid indefinitely without colliding with the human. 

This objective can be reduced to solving the satisficing problem in a quantitative game. 





==> Chapters/cav18/Section/Abstract.tex <==
%Quantitative specifications are used to determine the quality of software and hardware systems. 
%These specifications are typically represented as weighted logics, weighted automata, and the like. 
%Despite their application in determining quality of systems and in quantitative verification, in general, the study of quantitative specifications has typically been conducted from  a theoretical standpoint. 
%In this paper, we conduct an empirical study of quantitative inclusion for discounted-sum weighted automata, or \DS-inclusion in short. 

The problem of {\em quantitative inclusion} formalizes the goal of comparing quantitative dimensions between systems such as worst-case execution time, resource consumption, and the like. Such systems are typically represented by formalisms such as weighted logics or weighted automata. Despite its significance in analyzing the quality of computing systems, the study of quantitative inclusion has mostly been conducted from a theoretical standpoint. In this work, we conduct the first empirical study of quantitative inclusion for discounted-sum weighted automata (\DS-inclusion, in short). 

Currently, two contrasting approaches for \DS-inclusion exist: the linear-programming based \cct{DetLP}  and the purely automata-theoretic \cct{BCV}.
Theoretical complexity of \DetLPt is exponential in time and space while of \BCVt is \cct{PSPACE}-complete. All practical implementations of \cct{BCV}, however, are also exponential in time and space. Hence, it is not clear which of the two algorithms renders a superior implementation.

In this work we present the first implementations of  these algorithms, and perform  extensive experimentation to compare between the two approaches. Our empirical analysis shows how the two approaches complement each other. This is a nuanced picture that is much richer than the one obtained from the theoretical study alone. 
%Thereby, emphasizing on the importance of complementing theoretical advances with empricial analysis. 

%we present \cct{QuIP} that improves upon practical shortcomings of \cct{BCV}, in the process also improving its in-practice complexity via the construction of a new and compact comparator. 


%Recent developments have shown that the discounted-sum inclusion problem (DS-inclusion, in short) is $\cc{PSPACE}$-complete.

%While efficient solvers exist for other $\cc{PSPACE}$-complete problems, such as (qualitative) equivalence, no tool exists for DS-inclusion. 

%In this paper, we present the first solver for DS-inclusion. Our tool $ \QuantIP $ incorporates algorithmic improvements to the existing decision procedures. Empirical analysis of $\QuantIP$ on randomly-generated and fixed benchmarks show that $\QuantIP$ scales up to inputs with few hundreds of states each. 




==> Chapters/cav18/Section/AlgImprove.tex <==
A thorough analysis of the $\BCV$ algorithm shows that it can quickly become intractable as the number of states of the input weghted-automata increases (Lemma~\ref{Lemma:SizeBCV}, Corollary~\ref{coro:TransDensityBCV}).
In this section, we describe our algorithm $\QuantIP$ that incorporates algorithmic modifications to $\BCV$ framework to acheive tighter bounds on the size of inputs to the qualitative-inlcusion step to make discounted-sum inlcusion more scalable. 
We also describe implemenation details of our tool $\QuantIP$.


\begin{algorithm}[t]
	\caption{ $\QuantIP(P,Q, d)$, Is $P \subseteq_d Q$?}
	\label{Alg:DSInclusion}
	\begin{algorithmic}[1]
		\STATE \textbf{Input: } Weighted automata $P$ and $Q$, and 
		rational-valued discount-factor $d>1$
		\STATE \textbf{Output: } $\mathsf{True}$ if $P \subseteq_d Q$, $\mathsf{False}$ otherwise
		
		\STATE $\mu \leftarrow \mathsf{MaxWt}(P, Q)$ \label{alg-line:maxWt}
		\STATE $\A_d \leftarrow \mathsf{MakeDSComparator}(\mu, d)$ \COMMENT{$\A_d$ accepts $(A,B)$ iff $\DSum{A}{d} < \DSum{B}{d}$} \label{alg-line:makeComp}
		\STATE $\hat{P} \leftarrow  \AugmentWtAndLabel(P)$ \label{alg-line:AugmentP}%\COMMENT{$\tau =  (s_1\xrightarrow{a} s_2) \in \delta_A$ becomes $\hat{\tau} = s_1\xrightarrow{a, wt_A(\tau), l_{\tau}} s_2$} 
		\STATE $\hat{Q} \leftarrow  \AugmentWt(Q)$  \label{alg-line:AugmentQ}%\COMMENT{$\tau =  (s_1\xrightarrow{a} s_2) \in \delta_A$ becomes $\hat{\tau} = s_1\xrightarrow{a, wt_A(\tau)} s_2$} 
		
		
		
		
		\STATE $\hat{P}\times\hat{Q} \leftarrow \MakeProduct(\hat{P}, \hat{Q})$ \label{alg-line:Prod}
		
		% \STATE $\mu \leftarrow \MaxWt(P,Q)$ \label{alg-line:MaxWt}
		% \STATE $\A_f \leftarrow \MakeDS(f, \mu)$ \label{alg-line:MakeDS} 
		%\COMMENT{Accepts $(A,B)$ iff $f(A) \leq f(B)$}
		
		\STATE $\less \leftarrow  \Intersect(\hat{P}\times\hat{Q}, \A_{d} )$  \label{alg-line:Intersect}
		
		
		\STATE $\first \leftarrow \Project(\less)$ \label{alg-line:Project}
		\IF {$\hat{P} \equiv \first$} \label{alg-line:ensure1}
		
		{\RETURN $\mathsf{True}$} 
		\ELSE  {\RETURN $\mathsf{False}$}
		\ENDIF \label{alg-line:ensureLast}
		
	\end{algorithmic}
\end{algorithm}

\subsection{Algorithm details}
\label{Sec:QIPDetails}
Our algorithm $\QuantIP$ (Algorithm~\ref{Alg:DSInclusion}) takes as input two discounted-sum automata $P$ and $Q$, rational discont-factor $d>1$ and returns $ \mathsf{True}$ iff $P \subseteq_d Q$.  The algorithm $\QuantIP$ is based on verifying if every run of $P$ is diminished. 
$\QuantIP$ is split into three major steps: First, the construction of the discounted-sum comparator (Line~\ref{alg-line:maxWt}-Line~\ref{alg-line:makeComp}); second , construction of all B\"uchi automata
$\first$ that consists of all diminished runs of discounted-sum automata $P$ (Line~\ref{alg-line:AugmentP}-Line~\ref{alg-line:Project}); and lastly, qualitative-equivalence between 
disambiguated runs of discounted-sum automata $P$, $\hat{P}$ and its diminished runs $\first$ (Line~\ref{alg-line:ensure1}-Line~\ref{alg-line:ensureLast}). 

The first and last steps of $\QuantIP$ are straightforward. Procedure $\mathsf{MakeDSComparator}$ implements the discounted-sum comparator $\A_d$ as described in~\cite{BCVLICS17}, with discount-factor $d$ and maximum bound $\mu$ on the integer sequences, where $\mu$ is the maximum weight along transitions in both input discounted-sum automata $P$ and $Q$. 
$\A_d$ accepts $(A,B)$ iff $\DSum{A}{d} < \DSum{B}{d}$
This implementation results in a discounted-sum comparator with $\O(\frac{\mu^2}{d})$ states and $\O(\mu^6/d^2)$ transitions. While the theoretical upper-bound on transition density of the comparator $\delta_d$ may seem very high i.e $\O(\mu^4d)$, in practice we observe much tighter bounds. (TO ADD TO APPENDIX). The last step of performs qualitative-equivalence  between $\hat{P}$, which is of the same size as $P$, and $\first$. 

\subsubsection{Construction of $\first$}
\label{Sec:FirstConstruction}
It is  in the construction of $ \first$ where our algorithm $\QuantIP$ differs from $\BCV$.  Here we explain our procedure for construction of $\first $ (Algorithm~\ref{Alg:DSInclusion}, Line~\ref{alg-line:AugmentP}-Line~\ref{alg-line:Project}), and contrast it with $\BCV$'s method. 

For a discounted-sum automata $M$, procedure $\AugmentWt$ associates weight-sequences of words with them. It converts $M$  to  a B\"uchi automata $\hat{M}$ s.t. if word $w \in M$ has a run $\rho \in M$ with weight $wt_{\rho}$, then the word $\hat{w} = (w, wt_{\rho}) \in \hat{M}$. This can be easily acheived by extending the alphabet of $M$ with weights i.e. convert every transition $\tau = (p, a, q)\in M$ with weight $wt$ to transition $\hat{\tau} = (p, (a, wt), q) \in \hat{M}$.
Similarly, $\AugmentWtAndLabel$ constructs B\"uchi automata $\hat{M}$ from discounted-sum automata $M$ s.t. in addition to  associating their weight-sequences to words, $\hat{M}$ also disambiguates between different runs of the same word. Specifically, it converts every transition $\tau = (p, a, q) \in M$ with weight $wt$ to transition $\hat{\tau} = (p, (a, wt, i), q) \in \hat{M}$, where $i$ is a unique number assigned to every transition of $M$.
Note that procedure $\AugmentWt$ and $\AugmentWtAndLabel$ extend the alphabet size of $\hat{M}$ by a factor of $\mu$ and $\mu\cdot\tau_M$ respectively, where $\mu$ is the maximum weight on transitions on $M$ and $\tau_M$ is the number of transitions in $M$.  


Procedure $\MakeProduct$ takes as input the augmented B\"uchi automata $\hat{P}$ and $\hat{Q}$, and returns their product s.t. transitions $ \tau_P  = (p_1, (a_1, wt_1, i ), q_1) \in \hat{P}$ and transitions $\tau_Q  = (p_2, (a_2, wt_2), q_2)\in \hat{Q}  $ combine to form transition $\tau_{P}\times\tau_{Q} = ((p_1, p_2),(a, wt_1, wt_2, i),(q_1, q_2)) \in \MakeProduct(\hat{P}\times\hat{Q})$ iff $a_1 = a_2$.
Therefore, $\hat{w} = (w, wt_1, wt_2, id) \in \hat{P}\times\hat{Q}$ iff $(w, wt_1, id) \in \hat{P}$ and $(w, wt_2) \in \hat{Q}$. In other words, $\hat{w} = (w, wt_1, wt_2, id) \in \hat{P}\times\hat{Q}$ iff the run $\rho \in P$ of word $w$ is uniquely identified by $id$ and its weight-sequence in $P$ is given by $wt_1$. At the same time, the same word $w$ has a run in $Q$ with the weight-sequence $wt_2$. 
\begin{lemma}
\label{Lemma:Product}
Word $\hat{w} = (w, wt_1, wt_2, id) \in \hat{P}\times\hat{Q}$ iff word $w\in P$ and $w \in Q$ s.t. its runs have  weight-sequences are $wt_1$ and $wt_2$ in $P$ and $Q$ respectively. This run of $w \in P$ is uniquely identified by $id$. 
\end{lemma}
Our objective is to find words  those word $ (w, wt_1, wt_2, id) \in \hat{P}\times \hat{Q}$ s.t. $\DSum{wt_1}{d}< \DSum{wt_2}{d}$. The discounted-sum comparator $\A_f$ enables just that. 
However, note that the alphabet of $\hat{P}\times\hat{Q}$ is of the form $(a, wt_1, wt_2, i) $ while that of $\A_f$ is of the form $(wt_1, wt_2)$. Since their alphabets are not compatible, standard interseciton cannot be applied here. An easy work-around here is to extend the alphabet of $\A_f$ to match that of $\hat{P}\times\hat{Q}$. Since the alphabet of every transition of $\A_f$ will have to be extended, this leads to an increase in number of transitions of $\A_f$ by a factor of $|\Sigma|\cdot  \tau_P$, where $\Sigma$  and $\tau$ are the  alphabet and total number of transitions of $P$. Subsequently, number of transitions in $\less$ also blows-up by the same factor. 

Procedure $\Intersect$ prevents this blow-up. Intuitively, instead of extending alphabet of $\A_f$, it ignores the extra alphabets of $\hat{P}\times\hat{Q}$, and then performs their naive intersection. Once this is complete, it adorns the resulting transitions back with the extra-alphabets. 

//DESCRIPTION OF $\Intersect$

\begin{lemma}
Let $S$ and $T$ be B\"uchi automata over the alphabet $\Sigma_1\times\Sigma_2\times\Sigma_3\times\Sigma_4$ and $\Sigma_2\times\Sigma_3$ respectively. 
Let $U = \Intersect(S, T) $. Then
\begin{itemize}
	\item $w  = (w_1, w_2, w_3, w_4)$ iff $w \in S$ and $(w_2, w_3)\in T$.
	\item Let $s_S$, $\tau_S$ and$ s_T$, $\tau_T$ denote the number of states and transitions in S and T respectively. Then the number of states and transitions of $U$ are $\O(s_Ss_T)$ and $\O(\tau_S\tau_T)$.
\end{itemize}

\end{lemma}

\subsubsection{Analysis of $\first$}
\label{Sec:FirstAnalysis}

\begin{lemma}
	\label{Lemma:SizeQIP}
	Let $s_P$, $s_Q$, $s_d$ denote number of states in $P$, $Q$ and $\A_d$ respectively. Similarly, let $\tau_P$, $\tau_Q$, $\tau_d$ denote number of transitions in $P$, $Q$ and $\A_d$ respectively. Let $\mu$ and $\Sigma$ denote maximum weight and the alphabet size of the input discounted-sum automata. 
	
	Number of states in $ \hat{P} $ and $ \first $ are $ s_p $ and $\O(s_P \cdot s_Q \cdot s_d)$ respectively. 
	Number of transition in  $ \hat{P} $ and $ \first $ are $\tau_P$ and $\O(\mu^2\cdot \tau_P \cdot \tau_Q \cdot \tau_d\cdot \Sigma)$ respectively.
	(Check)
\end{lemma}
\begin{corollary}
	\label{coro:TransDensityQIP}
	Let $s_P$, $s_Q$, $s_d$ denote the number of states of weighted automata $P$ and $Q$ and comparator $\A_d$ respectiely, and $\delta_P$, $\delta_Q$ and $\delta_d$ be their transition densities. 
	
	Transition density of $\first$ is $\O(\delta_P \delta_Q \delta_d  )$.
\end{corollary}
	
\subsubsection{Contrast with $\BCV$}
\label{Sec:ContrastWithBCV}








\subsection{Algorithm analysis}
\label{Sec:QIPAnalysis}


\subsection{Implementation details}

 


==> Chapters/cav18/Section/Discussion.tex <==
\section{Future work and conclusions}
\label{Sec:Discussion}



==> Chapters/cav19/Section/abstract.tex <==

{\em Discounted-sum inclusion} (DS-inclusion, in short) formalizes the goal of comparing quantitative dimensions of systems such as cost, resource consumption, and the like, when the mode of aggregation for the quantitative dimension is discounted-sum aggregation. {\em Discounted-sum comparator automata}, or \emph{DS-comparators} in short,  are B\"uchi automata that read two infinite sequences of weights synchronously and relate their discounted-sum. Recent empirical investigations have shown that while DS-comparators enable competitive algorithms for DS-inclusion, they still suffer from the scalability bottleneck of B\"uchi operations. 

Motivated by the connections between discounted-sum and B\"uchi automata, this paper undertakes an investigation of language-theoretic properties of DS-comparators in order to mitigate the challenges of B\"uchi DS-comparators to achieve improved scalability of DS-inclusion.  Our investigation uncovers that DS-comparators possess safety and co-safety language-theoretic properties. As a result,  they enable reductions based on subset construction-based methods as opposed to higher complexity B\"uchi complementation, yielding tighter worst-case complexity and improved empirical scalability for DS-inclusion.



==> Chapters/cav19/Section/functional.tex <==
\subsection{Functional-like automata}
\label{Sec:Functional}

A {\em weighted $\omega$-automaton} over infinite words is {\em functional} if any two  runs on the same word have the same weight~\cite{filiot2012quantitative}.
A functional weighted automata is helpful since despite being non-deterministic, they can be  used in place of deterministic weighted automata to obtain algorithms that do not incur the blow-up caused by non-deterministic. 
The polynomial time algorithm for quantitative inlcusion requiring that the right-hand side input be a deterministic weighted automata~\cite{chatterjee2010quantitative}  also works when the right-hand side input is a functional weighted automata. The drawback of functional weighted automata, though, is that decision procedures converting non-deterministic to equivalent functional weighed automata or determining if a given weighted automata is also functional are typically expensive and/or are catered by non-generic algorithms~\cite{filiot2012quantitative}. 

In this section, we introduce a functional-like automata that simulates a functional automata, and design a generic comparator-based algorithms to construct a functional-like automata from a weighted automata for $\omega$-regular aggregate functions.  We show that the resulting functional form automata possess safety or co-safety properties when the comparator also posseses co-safety or safety properties, respectively. In addition, the algoritm is able to utilitze benefits of safety/co-safety comparators to construct smaller functional-like automata than with general $\omega$-regular comparators. 
\begin{definition}[Functional-like automata]
	A B\"uchi automata is a {\em functional-like automaton} $\A$ over alphabet $\Sigma\times \N$ for a weighted automaton $\mathcal{W}$ with aggregate function $f:\N^\omega \rightarrow \Re $ over alphabet $\Sigma$ if 
	$(w, c) \in \L(\A) $ iff $wt(w) = f(c)$ in $\mathcal{W}$.
\end{definition}
A run $\rho_w$ of a word $w$ in weighted automata $B$ is said to be {\em dominated} by another run $\sigma_w$ of the same word $w$ in $B$ if $wt(\rho_w) < wt(\sigma_w)$.
Therefore, the weight of a words in a weigted automata are given by the runs that are not dominated by any other run in the weighted automata. 
Extracting these non-dominated runs forms the key idea behind the generic algorithm for constructing functional-like automata for weighted automata by extracting all non-dominated runs from the weighted-automata. 

The algorithm proceeds by constructing a B\"uchi automata with transitions ($s_1, s_2, c_1)\xrightarrow{a, wt_1, wt_2} (t_1, t_2, c_2)$, where $s_i \xrightarrow{a, wt_i} t_i$ is a transition in the annotated automata for the input weighted automata, and $c_1 \xrightarrow{wt_1, wt_2} c_2$ is a transition in the compartor $\A^\mu_<$. A state in the B\"uchi automata is accepting if $c_i$ is an accepting state in the comparator. It is easy to see that this B\"uchi autoamta will accept a word $(w, wt_1, wt_2) $ iff run of $w$ with weight sequence $wt_1$ is dominated by another run of $w$ with weight sequence $wt_2$ in the weighted automata. A projection of this B\"uchi automata on the first two components returns an automaton that accepts $(w,wt)$ iff word $w$ with weight sequence $wt$ is dominated in the weighted-automata, denoted by $\first$. 
$\first$ can be constructed by taking the produce of the annotated automata with itself, and intersection of this product with the comparator. 
The intersection of the annotated automata of the input weighted autoamta with $\ol{\first}$ results in the desired functional-like automata. 
Since this algorithm is closely inspired by the algorithm for quantitative inclusion with $\omega$-regular aggregate functions presented in~\cite{BCVFoSSaCS18}, its details have been deferred to the supplemental material. 

%This forms the key idea behind a generic algorithm for constructing functional-like automata for weighted-automata with an $\omega$-regular aggregate function. The algorithm proceeds by finding  all runs of the form $(w,wt)$, where $w$ is a word and $wt$ is its weight sequence, that are dominated by another run of the same word. Owing to the $\omega$-regular comparator, these dominated runs of the form $(w,wt)$ result in a B\"uchi automata. Finally, the removal of domianted runs from the weighted-automata via B\"uchi complementation results in its functional-form automata. 


%The wight of a word in a weighted autoamta is determined by those runs which is not domianted by any other run of the same word in the weighted automata. The key idea behind construction a functional automata from a weighted automata is by finding an automaton for all such runs. We proceed by finding an automaton for all dominated runs, and then complementing it to find all non-dominated runs or the functional automata equivalent of the input. 

\begin{lemma}
\label{lem:FunctionalGeneral}
Let $B$ be a weighed automata and $\A^{\mu}_<$  be the $\omega$-regular comparator for its aggregate function. 
The functional-like automata for B consists of $2^{\O( \log B + |B|^2\cdot |\A^\mu_<|\cdot \log(|B|\cdot |\A^\mu_<|)) }$ states. 

% the size of the functional automata form of $B$ generated from $\Func{B}$ is $|B|\cdot 2^{\O(|B|^2\cdot |\A^\mu_<|\cdot \log(|B|^2\cdot |\A^\mu_<|))}$.
\end{lemma}
$\first$ is formed by a product between $B$ with itself and the comparator $\A^\mu_<$, already resulting in $|B|\cdot \A^\mu_<$ states. B\'uchi complementation results in a $2^{n\log n }$ blow-up, when $n$ is the total number of states. The final intersection with $B$ results in an automata consisting of $2^{\O( \log B + |B|^2\cdot |\A^\mu_<|\cdot \log(|B|\cdot |\A^\mu_<|)) }$ states.

\subsubsection{With safety/co-safety comparator for $\A_<^\mu$}

In this section we study the impact of safety/co-safety comparators in constructing the functional-like automata. In each case, we show that complex B\"uchi complementation can be replaced by simpler subset construction techniques to acheive a funcitonal-like automata with fewer states. 
 
\paragraph{Safety compartor} 
First of all, annotated automata is a safety property since all its states are accepting states. Safety properties are closed under product and intersection. When the comparator is a safety property, $\first$ is also a safety property. 
%First of all, it is easy to show that product of annotated automata $\hat{B}$ with itself is a safety property, since all states are aceepting states. As a result, when the comparator automata $\A^\mu_<$ is a safety automata, $\first$ obtained by an intersection of the product of annotated autoamta with the comparator is also a safety property. 
Therefore, its complementation $\ol{\first}$ is obtained by subset construction, resulting in a comparatively lower $2^n$ blow-up,  and flipping the accepting and non-accepting states. 

\begin{lemma}
	\label{lem:FunctionalSafety}
	Let $B$ be a weighed automata and $\A^{\mu}_<$  be a safety comparator for  an aggregate function. 
	The functional-like automata for $B$ consists of $2^{\O( \log |B| + |B|^2\cdot |\A^\mu_<|) }$ states. 
\end{lemma}


\paragraph{Co-safety comparator}
The intersection of a safety property with a co-safety property results in a weak-B\"uchi automata (Lemma~\ref{Lem:IntersectSafetyAndCo}. As a result, when the comparator is a co-safety property, since the  product of annotated automata with itself is a safety property, $\first$ is a weak-B\"uchi automata. Complementation of a weak-alternating automata results in an $n\cdot 2^n$ blow-up: It is slightly more than complementing a safety property but still lower than a full-fledged B\"uchi complementation. In this case, the functional-like automata results in $2^{\O( \log |B| + \log |\A^\mu_< | + |B|^2\cdot |\A^\mu_<|) }$ states. 

Upon closer analysis, we show that one can instead construct an over-approximation of $\first$,  such that the over-approximation is a co-safety property and the intersection of the annotated automata with its complement results in a functional-form of the weighted automata. 
\textbf{TODO}








==> Chapters/cav19/Section/safety.tex <==
\section{Safety and co-safety comparators for discounted-sum}
\label{Sec:Safety}
%Earlier developments in discounted-sum comparators show that discounted-sum comparators are regular iff the discount-factor is an integer. 
This section delves deeper into the language-theoretic properties (safety and co-safety) of DS-comparison languages and their comparators. 
%In particular, we explore safety and co-safety properties of DS-comparison languages. 
This section begins with formal definitions of safety/co-safety comparison langauges and comparators (\textsection~\ref{Sec:SafeCoSafeDef}), and then explores them for the discounted-sum aggregate function with rational (integer and non-integer) discount-factors (\textsection~\ref{Sec:DS}). 

%



%The central contribution of this section is that DS-comparison languages are safety/co-safety languages for arbitrary discount-factors, and DS-comparator are safety/co-safety automata for integer discount-factor. Finally, we use these language-theoretic properties to propose {\em compact deterministic} constructions for DS-comparator with integer discount-factor that even match their existing non-deterministic constructions in number of states. 



\subsection{Safety and co-safety comparison languages and comparators}
\label{Sec:SafeCoSafeDef}
Safety and co-safety comparison languages and comparators are defined as: 
\begin{definition}[Safety and co-safety comparison languages]
Let $\Sigma$ be a finite set of natural numbers, $f:\N^{\omega}\rightarrow \mathbb{R}$ be an aggregate function, and $R  \in \{\leq, <, \geq, >, =, \neq\}$ be an inequality relation. 
A comparison language over $\Sigma\times\Sigma$ for aggregate function $f$ and relation $R $ is said to be a safety comparison language or a co-safety comparison language if it is a safety or co-safety language. 
\end{definition}
%By duality of safety and co-safety languages, the comparison language for strict inequality is  safety iff comparison language for non-strict inequality is  co-safety, and vice versa.

\begin{definition}[Safety and co-safety comparators]
Let $\Sigma$ be a {finite set} of natural numbers,  $f:\N^{\omega}\rightarrow \mathbb{R}$ be an aggregate function, and $R  \in \{\leq, <, \geq, >, =, \neq\}$ be an inequality relation. 
A comparator for aggregate function $f$ and relation $R$ is a {\em safety comparator} or {\em co-safety} comparator for $f$ with $R$ if its language is  safety or co-safety, respectively.

%A {\em safety comparator} or {\em co-safety comparator} for aggregate function $f$ with relation $R$ is a comparator  for $f$ and $R$ when its language is safety or co-safety, respectively.
\end{definition}
A safety comparator is {\em regular} if its language is  $\omega$-regular (equivalently, if its automaton is a safety automaton). 
Likewise, a co-safety comparator is {\em regular} if its language is  $\omega$-regular (equivalently, automaton is a co-safety automaton). 

By complementation duality of safety and co-safety automaton, we get that the comparator for an aggregate function $f$ for non-strict inequality $\leq$ is safety iff the comparator for $f$ for strict inequality $<$ is co-safety. 
%A safety and co-safety comparator is called {\em $\omega$-regular safety} and {\em $\omega$-regular co-safety} if its automaton is a safety and co-safety automaton, respectively.
By closure properties of safety and co-safety automata under intersection and union, regular safety comparator for non-strict inequality renders regular safety comparator for equality, and regular co-safety comparator for strict-inequality yields $\omega$-regular co-safety comparator for inequality $(\neq)$.

%Therefore, determining whether the comparison language for an aggregate function for any one inequality (and not equality) is safety or co-safety is sufficient to determine the status for all other inequalities and equality. 






\input{Section/dssafety}



==> Chapters/cav19/macro.tex <==
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{amsmath}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{graphicx}
%\usepackage{hyperref}
\usepackage[bookmarks=false]{hyperref}
\usepackage{listings}
\usepackage{makeidx}  % allows for indexgeneration
%\usepackage{smallsec} % self-style file
%\usepackage[compact]{titlesec}
\usepackage{subcaption}
\usepackage{url}
\usepackage{wrapfig}

%tikz package 
\usepackage[graphicx]{realboxes}
\usepackage{tikz}
\tikzset{elliptic state/.style={draw,ellipse}}
\usetikzlibrary{shapes,shapes.geometric,arrows,fit,calc,positioning,automata,}
\usetikzlibrary{automata,positioning}
\usepackage{tikz-qtree}
\usepackage{float}
\usepackage{floatflt}


\newcommand{\snote}[1]{\anotefrom{s}{#1}}


%General macros
\newcommand*{\cct}[1]{\textsf{#1}}
\newcommand*{\cc}[1]{\mathsf{#1}}
%\newcommand{\num}[3]{\#(#1)(#2[#3])}
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\Z}{\mathbb{Z}}
\renewcommand*{\L}{\mathcal{L}}
\renewcommand*{\O}{\mathcal{O}}
\newcommand{\ol}[1]{\overline{#1}}

%General math macros
\renewcommand*{\mod}[1]{|#1|}
\newcommand*{\ceil}[1]{\lceil #1 \rceil}
\newcommand*{\floor}[1]{\lfloor #1 \rfloor}

%General automata-theroetic notations
\newcommand*{\A}{\mathcal{A}}
\newcommand*{\Statess}{\mathit{S}}
\newcommand*{\State}{S}
\newcommand*{\Start}{s_I}
\newcommand*{\Final}{\mathcal{F}}
\newcommand*{\StartState}{{\mathit{Init}}}
\newcommand*{\AcceptingStates}{S_{acc}}
\newcommand*{\wt}{\mathit{wt}}
\newcommand*{\sink}{\mathsf{sink}}

%Safety macros
\newcommand*{\bad}[1]{\mathit{bad}(#1)}
\newcommand*{\pre}[2]{#1[#2]}
\newcommand*{\suf}[2]{#1[#2\dots]}
\newcommand{\gap}[1]{\mathsf{gap}(#1,d)}
\newcommand{\thresh}{\mathsf{T}}
\newcommand{\baut}[3]{\mathsf{bad}(#1, #2,#3)}

%macros for DS
\newcommand*{\DSum}[2]{\mathit{DS}({#1}, {#2})}
\newcommand*{\MaxC}{\mathit{maxC}}
\newcommand*{\MaxX}{\mathit{maxX}}


%macros for maximal
\newcommand*{\maximal}[1]{\mathsf{Maximal}(#1)}

%macros for counterexample

\newcommand*{\counter}[1]{\mathsf{Counterexample}(#1)}
\newcommand{\strict}{\mathsf{strct}}
\newcommand{\nstrict}{\mathsf{nstrct}}
\newcommand{\R}{\mathsf{inc}}


\newcommand{\todo}[1]{\textbf{TODO}{#1}}

\newcommand*{\LI}{\textsf{LI}}
\newcommand*{\LP}{\textsf{LP}}
\newcommand*{\DS}{\textsf{DS}}

==> Chapters/integergames/Section/lowerapproxcomparator.tex <==
\subsection{Comparator automata for lower approximation of DS with threshold value $v$}

We assume that the threshold value is  represented by the regular expression $v = v[0]v[1]\dots v[m](v[m+1]v[m+2]\dots v[n])^{\omega}$. By abuse of notation, we denote both the regular expression $ v[0]v[1]\dots v[m](v[m+1]v[m+2]\dots v[n])^{\omega}$ and the value $\DSum{v}{d}$ by $v$.


The comparator construction is similar to the one from earlier. 
The core idea is to use the inductive definition of approximate gap value (lower gap value and upper gap value) for the comparator construction. Since the approximate gap values are discrete, we use the lower gap values for states in the construction. To ensure that there are only finitely many states, we show that it is sufficient to consider a finite number of gap values only. 

We begin by showing that it is enough to look at finitely many values. 
For this we show that the comparison language with threshold $v$ for inequality $\leq $ is a safety language by proving that sequences that are not present in the language possess a bad prefix. 
We denote the comparison language for the lower approximation of discounted-sum withdiscount-factor $d= 1+2^{-k}$, precision $\varepsilon=2^{-p}$,  upper bound $\mu$, relation $\leq$ and threshold  $v$ by $\A^{\mu, d, \varepsilon}_{\leq v}$.


\begin{lemma}
\label{Lem:GapThresholdBad}
	Let $\mu$ and $d = 1+2^{-k}>1 $, precision $\varepsilon = 2^{-p}$ be the bound, discount-factor, and precision respectively.
	Let $W$ be a non-empty, bounded, finite weight-sequence.   
	Weight sequence $W$ is a bad-prefix of $\A^{\mu,d, \varepsilon}_{\leq v}$  iff 
	$\gapL{W} > \gap{\pre{v}{|W|}} +  \frac{1}{d}\cdot \DSum{\post{v}{|W|}}{d} - \frac{\mu}{d-1}$.
\end{lemma}	
\begin{proof}
We first establish the following: For all weight-sequences $X$ and integer $n> 0$
\[
\DSumL{X} = \frac{\gapL{X[n]}}{d^{n-1}} +\frac{1}{d^{n}}\cdot (\DSum{X[n\dots]}{d} - \DSum{\delta}{d})
\]
where $X[n\dots] = X_nX_{n_1}\dots$, and $\delta$ is an infinite non-negative rational-value weight-sequence bounded by the resolution $2^{-(p+k)}$.

From Lemma~\ref{lem:EquivGapAndApproxGapLow}, we know that there exists a rational-valued weight-sequence $U$ such that $\DSumL{X} = \DSum{U}{d}$. More specifically, the $i$-th element of $U$ i.e $U_i$ is equal to $X_i -\varepsilon_i$, where $0\leq \varepsilon_i < 2^{-(p+k)}$. Let $\varepsilon = \varepsilon_0\varepsilon_1\dots$, then $U = X - \varepsilon$.
%The same holds for weight-sequence $Y = X_n X_{n+1}\dots$. Let $V$ and $\delta$ be the corresponding weight-sequences. 
Furthermore we also know that for all $n> 0$, $\gapL{X[n]} = \gap{U[n]}$. Therefore, for all $n> 0$

\begin{align*}
    \DSumL{X} & = \DSum{U}{d} \\
    & = \frac{\gap{U[n]}}{d^{n-1}} + \frac{1}{d^n}\cdot \DSum{U[n\dots]}{d} \\
    & = \frac{\gapL{X[n]}}{d^{n-1}} + \frac{1}{d^n}\cdot \DSum{X[n\dots] - \varepsilon[n\dots]}{d} \\
    & =  \frac{\gapL{X[n]}}{d^{n-1}} + \frac{1}{d^n}\cdot (\DSum{X[n\dots]}{d}- \DSum{\delta}{d}), \text{ where } \delta = \varepsilon[n\dots]
\end{align*}


We show that if the condition holds, then $W$ is a bad prefix. 

Let $Y$ be an arbitrary weight sequence. Then 
$\DSumL{W\cdot Y} = 
\frac{\gapL{W}}{d^{n-1}} + \frac{1}{d^n}\cdot (\DSum{Y[n\cdots ]}{d} - \DSum{\delta[n\cdots]}{d}) = 
\frac{1}{d^{n-1}} \cdot (\gapL{W} + \frac{1}{d}\cdot (\DSum{Y[n\cdots ]}{d} - \DSum{\delta[n\cdots]}{d}))$. 
From the given condition, we get that 
$\DSumL{W\cdot Y} > 
\frac{1}{d^{n-1}} \cdot ( \gap{\pre{v}{|W|}} +  \frac{1}{d}\cdot \DSum{\post{v}{|W|}}{d} - \frac{\mu}{d-1} + \frac{1}{d}\cdot (\DSum{Y[n\cdots ]}{d} - \DSum{\delta[n\cdots]}{d})  )$.
The LHS is maximized when $\DSum{Y[n\cdots]}{d} = \frac{\mu\cdot d}{d-1}$ and $\DSum{\delta[n\cdot]}{d} = 0$.
Then 
$\DSumL{W\cdot Y} > 
\frac{1}{d^{n-1}} \cdot ( \gap{\pre{v}{|W|}} +  \frac{1}{d}\cdot \DSum{\post{v}{|W|}}{d}) = \DSum{v}{d} = v$. Therefore, $\DSumL{W\cdot Y} > v$ for an arbitrary weight sequence $Y$. Hence, $W$ is a bad prefix. 

Conversely, we prove that if $W$ is a bad prefix, then the condition holds. 
Therefore, for all weight sequences $Y$, $\DSumL{W\cdot Y} > v$ iff $\frac{\gapL{W}}{d^{n-1}} + \frac{1}{d^n}\cdot (\DSum{Y - \delta[n\cdots]}{d}) > \frac{1}{d^{n-1}}\cdot (\gap{v[n]} + \frac{1}{d}\cdot \DSum{v[n\cdots]}{d})$. 
By  cancelling the common denominator we get that $\gapL{W} + \frac{1}{d}\cdot \DSum{Y - \delta[n\cdots]}{d} > \gap{v[n]} + \frac{1}{d}\cdot \DSum{v[n\cdots]}{d}$. 
By rearrangement of terms, $\gapL{W} - \gap{v[n]} > \frac{1}{d}\cdot (\DSum{Y - \delta[n\cdots]}{d} + \DSum{v[n\cdots]}{d})$. The LHS is maximized if $\DSum{Y}{d} = \frac{\mu\cdot d}{d-1}$ and $\DSum{\dela[n\cdots}{d} = 0$. Therefore, we get that $\gapL{W} - \gap{v[n]} > \frac{\mu}{d-1} + \frac{1}{d}\cdot \DSum{v[n\cdots]}{d}$.

\end{proof}

We define {\em very-good prefixes} for $\A^{\mu,d}_\leq$: A finite and bounded weight-sequence $W$ is a {\em very good} prefix for language of $\A^{\mu,d}_\leq$ if
for all infinite, bounded extensions of $W$ by $Y$,  $\DSum{W\cdot Y}{d}\leq v$. 
A proof similar to Lemma~\ref{Lem:GapThresholdBad} proves an upper bound for the recoverable gap of very-good prefixes of $\A^{\mu,d,\varepsilon}_{\leq v}$:

\begin{lemma}
	\label{Lem:GapThresholdVeryGood}
	Let $\mu$ and $d>1 $ be the bound and discount-factor, resp.
	Let $W$ be a non-empty, bounded, finite weight-sequence.   
	Weight sequence $W$ is a very good-prefix of $\A^{\mu,d,\varepsilon}_{\leq v}$ iff $\gap{W-\pre{v}{|W|}} \leq \frac{1}{d}\cdot \DSum{\post{v}{|W|}}{d} + \frac{\mu}{d-1} + d\cdot\varepsilon$.
\end{lemma}


\begin{theorem}
\label{thrm:regularWithVal}
Let $\mu>0$ be the upper bound. Let $d >1$ be the integer discount factor. Let the threshold $v$ be such that $-\mu\cdot\frac{d}{d-1} < v < \mu\cdot\frac{d}{d-1}$. Let $v$ have a finite regular expression in the alphabet. 
Then the DS comparator automata with threshold value $v$ is an $\omega$-regular comparator. 
\end{theorem}
\begin{proof}



Let $\mu$ be the upper bound, and $d>1$ be the integer discount factor. 
Let the threshold value can be represented by the regular expression $v = v[0]v[1]\dots v[m](v[m+1]v[m+2]\dots v[n])^{\omega}$.
%Let $\thresh = \frac{\mu}{d-1}$ be the state-threshold value. 

For $i \in \{0,\dots,n\}$, let $\mathsf{U}_i = \frac{1}{d}\cdot \DSum{\post{v}{i}}{d} + \frac{\mu}{d-1}$.

For $i \in \{0,\dots,n\}$, let $\mathsf{L}_i = \frac{1}{d}\cdot \DSum{\post{v}{i}}{d} - \frac{\mu}{d-1}$.


The finite-state automata $\baut{\mu}{d}{\leq} = (\State, \Start, \Sigma, \delta, \Final)$ is defined as follows:

\begin{itemize}


\item States $\State = \bigcup_{i=0}^n S_i \cup \{\mathsf{bad}, \mathsf{veryGood}\}$ where 

$S_i = \{(s, i) | s \in \{\floor{\mathsf{L}_i}+1, \dots , \floor{\mathsf{U}_i} \}\} $

\item Initial state $\Start = (0,0)$, Accepting states $\Final = S\setminus\{\mathsf{bad}\}$
\item Alphabet $\Sigma = \{-\mu, -\mu+1,\dots, \mu-1, \mu\}$
\item Transition function $\delta\subseteq \State \times \Sigma \rightarrow \State$ where $(s,a,t) \in \delta$ then:
	\begin{enumerate}
	\item \label{Trans:SelfLoop} If $s \in \{\mathsf{bad}, \mathsf{veryGood}\}$, then $t = s$ for all $a \in \Sigma$
	\item If $s$ is of the form $(p,i)$, and $a \in \Sigma$
		\begin{enumerate}
		\item \label{Trans:leq} If $d\cdot p+a-v[i] > \floor{\mathsf{U}_i}$, then $t = \mathsf{bad}$
		\item \label{Trans:geq} If $d\cdot p+a -v[i]\leq \floor{\mathsf{L}_i}$, then $t = \mathsf{veryGood}$
		\item \label{Trans:IntState} If $\floor{\mathsf{L}_i} <  d\cdot p+a -v[i] \leq \floor{\mathsf{U}_i}$, 
		\begin{enumerate}
		    \item If $i == n$, then $t = (d\cdot p+a - v[i], m+1)$
		    \item Else, $t = (d\cdot p+a - v[i], i+1)$
		\end{enumerate}
%		\item \label{Trans:IntState} If $\floor{-\thresh} +1 \leq d\cdot s+a \leq \floor{\thresh}$, then $t = d\cdot s+a$
		
		\end{enumerate}
	
	\end{enumerate}
\end{itemize}

%\todo{ Complete proof argument}

\end{proof}

\begin{corollary}
\label{coro:regularWithVal}
Let $\mu>0$ be the upper bound. Let $d >1$ be the integer discount factor. Let the threshold $v$ be such that $-\mu\cdot\frac{d}{d-1} < v < \mu\cdot\frac{d}{d-1}$. Let $v$ have a finite regular expression in the alphabet given by $v = v[0]v[1]\dots v[m](v[m+1]v[m+2]\dots v[n])^{\omega}$. 
Then the DS comparator automata with threshold value $v$ is a regular safety/co-safety automata with $\O(\frac{\mu\cdot n}{d-1})$ states. 
\end{corollary}



==> Chapters/integergames/Section/lowerapproximation.tex <==

\subsection{Lower approximations of discounted-sum over infinite sequences}

\label{Sec:ApproxDSLower}

In this section, we define aggregate functions that can approximate discounted-sum when the discount-factor $d\rightarrow 1^+$. Specifically, we define two aggregate functions, one that bounds the discounted-sum from above and the other does the same from below, within a given desired precision factor. To this end,  we define {\em lower and upper recoverable gap}, and use them to define the {\em lower and upper approximations of discounted-sum}.

We are motivated by the notions of recoverable gap and its relation to {\em exact} discounted-sum.
The discounted-sum of an infinite and bounded weight-sequence can be defined in terms of the {\em recoverable gap} of its finite prefixes, as follows:
Let integer $\mu>0$ be the bound on weight-sequences. 
Let rational-number $d >1$ be the discount-factor. 
%Let $A$ be a finite and bounded weight-sequence. 
The {\em recoverable gap} of a finite, bounded, weight-sequence $W$ and discount-factor $d$, denoted by $\gap{W}$, is 0 if $|W|=0$ and $\gap{U\cdot u} = d\cdot \gap{U} + u$ if $W = U\cdot u          $.
Let $A[n]$ denote the $n$-length prefix of infinite and bounded-weight sequence $A$.
Intuitively, the recoverable gap of a finite weight-sequence is the normalized discounted-sum of the finite weight-sequence. Then, one can prove that $\lim_{n\rightarrow\infty}\frac{\gap{A[n]}}{d^{n-1}} \rightarrow \DSum{A}{d}$.




But first we introduce some notation. 
%Let integer $\mu>0$ be the bound on weight-sequences. 
Let the non-integer discount-factor $d>1$ be give by $1+2^{-k}$ for a rational-value $k>0$. 
Let the {\em precision} be given by $2^{-p}$ for rational-value $p> 0$. We define {\em resolution} as $r = 2^{-(p+k)}$. 
    
For a real number $x \in \Re$, we define $\roundL{x}$ rounds-up value $x$ to the largest integer multiple of the resolution that is smaller than or equal to $x$.
%and smallest integer multiple of the resolution. 
Formally, $\roundL{x} = i\cdot 2^{-(p+k)}$ such that $i \in \Z$ is the largest integer such that $i\cdot r \leq x$. 
Clearly, 

\begin{lemma}
\label{lem:LowerRound}
Let $k,p >0$ be rational-valued parameters. Then,
for all real values $x\in \Re$, $0\leq x - \roundL{x} < 2^{-(p+k)}$.
\end{lemma}
%\begin{lemma}
%\label{lem:LowerRoundSum}
%Let $k,p >0$ be rational-valued parameters. Then,
%for all real values $x,y\in \Re$, $\roundL{x + y} \geq \roundL{x} + \roundL{y}$.
%\end{lemma}
%\begin{proof}
%Let $x = i\cdot 2^{-(p+k)} + x_r$ and $y = j\cdot 2^{-(p+k)} + y_r$ for integers $i$ and $j$ such that $\roundL{x} = i\cdot 2^{-(p+k)}$ and $\roundL{y} = j\cdot 2^{-(p+k)}$. Then $0 \leq x_r,y_r < 2^{-(p+k)}$. 
%So, $\roundL{x+y} = \roundL{(i+j)\cdot 2^{-(p+k)}  + x_r + y_r} \geq \roundL{x} + \roundL{y}$. 
%\end{proof}
\begin{lemma}
\label{lem:LowerRoundMonotone}
Let $k,p >0$ be rational-valued parameters. Then,
for all real values $x,y\in \Re$ s.t. $x\geq y$, $\roundL{x} \geq \roundL{y}$.
\end{lemma}
%\begin{lemma}
%\label{lem:LowerRoundMonotoneOnPrecision}
%Let $k,p_1,P_2 >0$ be rational-valued parameters such that $p_1>p_2$. 
%Then for all real value $x\in \Re$, 
%\end{lemma}
We define the {\em lower approximation of recoverable gap} of a finite and bounded weight sequence $W$, discount-factor $d = 1+2^{-k}$ and precision $2^{-p}$, denoted $\gapL{W}$, is 0 if $|W| = 0$ and $\gapL{U\cdot u} =  \roundL{d\cdot \gapL{U} + u}$ if $W  = U\cdot u$.



Motivated by $\lim_{n\rightarrow\infty}\frac{\gap{W[n]}}{d^{n-1}} \rightarrow \DSum{W}{d}$, where $W[n]$ is the $n$-length prefix of infinite weight sequence $A$, we attempt to define a notion of lower approximation of discounted-sum in terms of lower approximation of  recoverable gap. Specifically, we want to define $\DSumL{W}$ as  $\lim_{n\rightarrow\infty}\frac{\gapL{W[n]}}{d^{n-1}}$. However, to make this definition valid, we first need prove that $\frac{\gapL{W[n]}}{d^{n-1}}$ converges as $n\rightarrow\infty$.
We proceed by proving that for all infinite and bounded integer sequences $W$, there exists an infinite and bounded rational-number sequence $U$ such that for all $n>0$, $\gap{W[n]} = \gapL{U[n]}$ for $n$-length prefixes $W[n]$ and $U[n]$ of $W$ and $U$, respectively (Lemma~\ref{lem:EquivGapAndApproxGapLow}). Finally, we use convergence of $\frac{\gap{U[n]}}{d^{n-1}}$ as $n\rightarrow\infty$ to prove the convergence of  $\frac{\gapL{W[n]}}{d^{n-1}}$ as $n\rightarrow\infty$, thereby proving the validity of our definition of $\DSumL{W}$.

\begin{lemma}
\label{lem:EquivGapAndApproxGapLow}
Let $d = 1+2^{-k}$ and $2^{-p}$ be the discount-factor and precision, for  rational numbers $k,p>0$. Let $\mu>0$ be the upper-bound.
Let $W$ be an infinite and bounded  weight-sequence. Then, there exists an infinite and bounded {\em rational number} weight-sequence $U$ such that for all $n>0$, $\gapL{W[n]} = \gap{U[n]}$, where $W[n]$ and $U[n]$ are $n$-length prefixes of $W$ and $U$, respectively. 
\end{lemma}

\begin{proof}
For sake of simplicity, we prove the result for {\em integer} weight-sequence first. %is an integer weight sequence. 

Let $W = W_0W_1W_2\dots$ such that for all $i\geq 0$, $W_i \in \Z$ and $|W_i| < \mu$. We will construct infinite and bounded rational sequence $U$ inductively. 

Base case: Consider the 1-length prefix of $W$, $W[1] = w_0$. By definition,  $\gapL{W[1]} = \roundL{W_0} = w_0$ for a rational-number $w_0$. From Lemma~\ref{lem:LowerRound}, we know that $0< W_0 - w_0 < 2^{-(p+k)}$. Therefore, since $W_0$ is an integer bounded by $\mu$, $w_0$ is a rational-number bounded by $\mu$ as well. 

We set $U_0$, the 0-th element of $U$, to be $w_0$. It is easy to see that $ \gap{U_0} = w_0 = \gapL{W[1]}$.

Inductive hypothesis: For an $n>0$, let there exist an $n$-length rational-number sequence $ U_0U_1\dots U_{n-1}$ bounded by $\mu$ such that for all $m\leq n$ it holds that $\gapL{W[m]} = \gap{U_0U_1\dots U_{m-1}}$.

Induction step: 
To prove the induction step, it is sufficient to show that the $n$-length bounded and rational-number weight-sequence $ U_0U_1\dots U_{n-1}$ from the induction hypothesis
can be extended by appending a rational-number $U_n$ bounded by $\mu$ such that 
$\gapL{W[n+1]} = \gap{U_0U_1\dots U_{n}}$ holds. 

By definition, $\gapL{W[n+1]} =\roundL{d\cdot \gapL{W[n]} + W_n}$. By definition of $\roundL{}$, we get that $\roundL{d\cdot \gapL{W[n]} + W_n} = d\cdot \gapL{W[n]} + W_n -\varepsilon_n$ when $\varepsilon_n$ is a rational-number such that $ 0\leq \varepsilon_n < 2^{-(p+k)}$. Therefore, we obtain that $\gapL{W[n+1]} = d\cdot \gapL{W[n]} + W_n -\varepsilon_n$. By induction hypothesis, we get that $\gapL{W[n+1]} = d\cdot \gap{U_0U_1\dots U_{n-1}} + W_n -\varepsilon_n$. Set $U_n = W_n -\varepsilon_n$. As reasoned in the base-case, we obtain that $U_n$ is rational number bounded by $\mu$. Therefore, $\gapL{W[n+1]} = \gap{U_0U_1\dots U_n}$.

Let $U$ be the infinite and bounded rational-number weight-sequence generated as defined above. Then  for all $n>0$, $\gapL{W[n]} = \gap{U[n]}$, where $W[n]$ and $U[n]$ are $n$-length prefixes of $W$ and $U$, respectively. 

Note that such a $U$ exists for all infinite and bounded-weight sequences $W$, even if $W$ is not an integer weight-sequence. The difference is that for a general rational number weight sequence if $W$ is bounded by $\mu$, then the $U$ will be bounded by $\mu+1$.
\end{proof}



\begin{corollary}
\label{cor:LimitExistsLower}
Let $d = 1+2^{-k}$ and $2^{-p}$ be the discount-factor and precision, for  rational numbers $k,p>0$. Let $\mu>0$ be the upper-bound.
Let $W$ be an infinite and bounded weight-sequence. 
Then  $\lim_{n\rightarrow\infty}\frac{\gapL{W[n]}}{d^{n-1}}$ exists, where W[n] is the $n$-length prefix of $ W$. 
\end{corollary}

\begin{proof}
We know from Lemma~\ref{lem:EquivGapAndApproxGapLow}, that there exists an infinite and bounded {\em rational number} weight-sequence $U$ such that for all $n>0$, $\gapL{W[n]} = \gap{U[n]}$, where $W[n]$ and $U[n]$ are $n$-length prefixes of $W$ and $U$, respectively. Therefore, $\frac{\gapL{W[n]}}{d^{n-1}} = \frac{\gap{U[n]}}{d^{n-1}}$. Since $\lim_{n\rightarrow\infty}\frac{\gap{U[n]}}{d^{n-1}}$ exists, we also get that  $\lim_{n\rightarrow\infty}\frac{\gapL{W[n]}}{d^{n-1}}$ exists and it is equal to $\DSum{U}{d}$.
\end{proof}

We have proven that the desired limit exists. Therefore, we can give the following valid definition for a {\em lower approximation of discounted-sum} of an infinite and bounded weight-sequence:

\begin{definition}{\rm [Lower approximation of discounted-sum]}
\label{def:ApproxDSLower}
Let $d = 1+2^{-k}$ and $2^{-p}$ be the discount-factor and precision, for  rational numbers $k,p>0$. Let $\mu>0$ be the upper-bound.
Let $W$ be an infinite and bounded weight-sequence. The {\em lower approximation of discounted-sum with discount-factor $d=1+2^{-k}$ and precision $2^{-p}$}, denoted by $\DSumL{W}$, is defined as $\lim_{n\rightarrow\infty}\frac{\gapL{W[n]}}{d^{n-1}}$, where $W[n]$ is the $n$-length prefix of $W$.
\end{definition}

For sake of brevity, we refer to {\em lower approximation of discounted-sum with discount-factor $d=1+2^{-k}$ and precision $2^{-p}$} by {\em lower approximation of discounted-sum}, and mention the parameters $k,p>0$ only when needed. 

Finally, we prove that the lower approximation of discounted-sum with discount-factor $d=1+2^{-k}$ and precision $2^{-p}$ is is within $2^{-p}\cdot d$ distance of the discounted-sum with the same discount-factor $d$ from below.

In the following, we provide results on the lower approximations of recoverable gap, and use it to define a lower approximation of discounted-sum. We define resolution sequences:
An $n$-length resolution sequence is the $n$-length sequence in which all elements are the resolution $r=2^{-(p+k)}$.
\begin{lemma}
\label{lem:LowerGapDifBounded}
Let $d = 1+2^{-k}$ and $2^{-p}$ be the discount-factor and precision, for  rational numbers $k,p>0$. Let $\mu>0$ be the upper-bound.
Let $W$ be a non-empty, finite and bounded weight-sequence. Then $0\leq \gap{W} - \gapL{W} < \gap{R}$, where $R$ is $|W|$-length resolution sequence. 
\end{lemma}
\begin{proof}
Base cases: $|W|=1$. Let $W = W_0$ for integer $W_0$ s.t $|W_0|\leq \mu$. Then $\gap{W} = \gapL{W} = W_0$. Then $\gap{W} = W_0$ and $\gapL{W} = \roundL{W_0}$. From Lemma~\ref{lem:LowerRound}, we get that $0\leq \gap{W} - \gapL{W} < 2^{-(p+k)} = \gap{R}$, where $R$ is the resolution sequence of length $1$.

Let the inductive hypothesis be that for all weight-sequences $W$ of length $n\geq1$,  it is true that $0\leq \gap{W} - \gapL{W} < \gap{R}$, where $R$ is $|W|$-length resolution sequence.

Induction step: We extend this result to weight-sequences of length $n+1$. Let $W$ be an $n+1$-length weight-sequence. Then $W = W[n] \cdot W_n$, where $W[n]$ is the $n$-length prefix of $W$ and $W_n$ is an integer s.t. $|W_n|< \mu$. 
%Then $\gap{W} - \gapL{W} = d\cdot \gap{W[n]} + W_n - \roundL{d\cdot\gapL{W[n]} + W_n }$.

We first show that $\gap{W} - \gapL{W}\geq 0$:
\begin{align*} 
& \gap{W} - \gapL{W} \\
= &  d\cdot \gap{W[n]} + W_n - \roundL{d\cdot\gapL{W[n]} + W_n }\\
& \text{ From Lemma~\ref{lem:LowerRoundMonotone} and the inductive hypothesis, we get} \\
\geq &     d\cdot \gap{W[n]} + W_n - \roundL{d\cdot\gap{W[n]} + W_n } \\
& \text{ From Lemma~\ref{lem:LowerRound}, we get the desired result} 
\end{align*} 

So,  $\gap{W} - \gapL{W} \geq 0$. Next, we show that $\gap{W} - \gapL{W} < \gap{R}$, where $R$ is the $|W|$-length resolution sequence. 
\begin{align*} 
& \gap{W} - \gapL{W} \\
= &  d\cdot \gap{W[n]} + W_n - \roundL{d\cdot\gapL{W[n]} + W_n }\\
& \text{ From Lemma~\ref{lem:LowerRound}, we get} \\
< &     d\cdot \gap{W[n]} + W_n - {(d\cdot\gapL{W[n]} + W_n)} + 2^{-(p+k)} \\
= &   d\cdot \gap{W[n]}  - {d\cdot\gapL{W[n]}} + 2^{-(p+k)} \\
& \text{ From the inductive hypothesis, we get} \\
< & d\cdot\gap{R'} + 2^{-(p+k)} \text{ where } R' \text{ is the } |W[n]|\text{-length resolution sequence} \\
= & \gap{R} \text{ where } R \text{ is the } |W|\text{-length resolution sequence}
\end{align*} 
Therefore, we have also proven that $\gap{W} - \gapL{W} < \gap{R}$, where $R$ is the $|W|$-length resolution sequence.
\end{proof}

\begin{theorem}
\label{thrm:ApproxDSLower}
Let $d = 1+2^{-k}$ and $2^{-p}$ be the discount-factor and precision, for  rational numbers $k,p>0$. Let $\mu>0$ be the upper-bound.
Let $W$ be an infinite and bounded weight-sequence. 
Then, $0\leq \DSum{W}{d} - \DSumL{W} < 2^{-p}\cdot d$.
\end{theorem} 
\begin{proof}
Let $R_n$ denote the $n$-length resolution sequence, and $R$ be infinite-length resolution sequence. From Lemma~\ref{lem:LowerGapDifBounded}, we know that for all $n>0$, 
\begin{align*}
&0\leq \gap{W[n]} - \gapL{W[n]} < \gap{R_n}\\
\iff & 0\leq \frac{(\gap{W[n]} - \gapL{W[n]})}{d^{n-1}} < \frac{\gap{R_n}}{d^{n-1}}\\
\iff &0\leq \frac{(\gap{W[n]}}{d^{n-1}} - \frac{\gapL{W[n]})}{d^{n-1}} < \DSum{R}{d} \\
&\text{Taking limit and by simplifying, we get} \\
\iff &0\leq \DSum{W}{d} - \DSumL{W} < 2^{-p}\cdot d
\end{align*}
\end{proof}
Lemma~\ref{lem:LowerGapDifBounded} and Theorem~\ref{thrm:ApproxDSLower} can be refined further when the weight-sequence are integers, and parameters $p,k>0$ are also integers. 


==> Chapters/integergames/Section/misc.tex <==
\section{Appendix}



\subsubsection{Lemma~\ref{lem:optimalplay}}
{\em
Let $l = l_1\cdot (l_2)^{\omega}$ represent  an integer cost sequence of a lasso, where $l_1$ and $l_2$ are the cost sequences of the head and loop of the lasso. Let $d = \frac{p}{q}$ be the discount factor. 
Then, $\DSum{l}{d}$ is a rational number with denominator at most ($p^{|l_2|} - q^{|l_2|})\cdot (p^{|l_1|})$.
}

\begin{proof}
The discounted sum of $l$ is given as follows:
\begin{align*}
    \DSum{l}{d} 
    = & \DSum{l_1}{d} + \frac{1}{d^{|l_1|}} \cdot(\DSum{(l_2)^\omega}{d})   \\
    = & \DSum{l_1}{d} + \frac{1}{d^{|l_1|}} \cdot \Big(\DSum{l_2}{d} + \frac{1}{d^{|l_2|}}\cdot \DSum{l_2}{d} + \frac{1}{d^{2\cdot|l_2|}}\cdot \DSum{l_2}{d}+ \dots\Big) \\
    & \text{Taking closed form expression of the term in the parenthesis, we get} \\
    = & \DSum{l_1}{d} + \frac{1}{d^{|l_1|}} \cdot \Big(\frac{d^{|l_2|}}{d^{|l_2|} -1 }\Big)\cdot \DSum{l_2}{d}  \\
    & \text{Let } l_2 = b_0b_1\dots b_{|l_2|-1} \text{ where } b_i \in \Z \\
    =  &\DSum{l_1}{d} + \frac{1}{d^{|l_1|}} \cdot \Big(\frac{d^{|l_2|}}{d^{|l_2|} -1 }\Big)\cdot \Big(b_0 + \frac{b_1}{d} + \dots + \frac{b_{|l_2|-1}}{d^{|l_2|-1}}\Big) \\
    =  &\DSum{l_1}{d} + \frac{1}{d^{|l_1|}} \cdot \Big(\frac{1}{d^{|l_2|} -1 }\Big)\cdot \Big(b_0\cdot d^{|l_2|} + {b_1}\cdot d^{|l_2|-1} + \dots + {b_{|l_2|-1}}{d}\Big) \\
    & \text{Expressing } d =\frac{p}{q} \text{, we get} \\
    = & \DSum{l_1}{d} + \frac{1}{d^{|l_1|}} \cdot \frac{q^{|l_2|}}{p^{|l_2|} - q^{|l_2|}}\cdot \Big(b_0 (\frac{p}{q})^{|l_2|} + \dots b_{|l_2|-1}\cdot \frac{p}{q}\Big) \\
    & \DSum{l_1}{d} + \frac{1}{d^{|l_1|}} \cdot \frac{1}{p^{|l_2|} - q^{|l_2|}}\cdot M, \text{ where } M \in \Z \\
    & \text{Expressing } d =\frac{p}{q} \text{ again, we get} \\
    = & \frac{1}{p^{|l_1|}} \cdot \frac{1}{p^{|l_2|} - q^{|l_2|}} \cdot N,  \text{ where } N \in \Z
\end{align*}
\end{proof}


\subsubsection{Theorem~\ref{thrm:vsquareiterations} [Zwick-Paterson's claim~\cite{zwick1996complexity}]}
{\em 
Let $G = (V, \init,E,\gamma)$ be a graph game. The number of iterations required by the value-iteration algorithm or the length of the finite-length game
to compute the optimal value $\opt$ is
\begin{enumerate}
    \item $\O(|V|^2)$ when discount factor $d\geq 2$, 
    \item $\O\Big(\frac{\log(\mu)}{d-1} + |V|^2\Big)$ when discount factor $1<d<2$.
\end{enumerate}
%can be computed from the optimal cost of an $O(|V|^2)$-length game. In other words, optimal value $W$ can be computed  from the aforementioned value-iteration algorithm in $\O(|V|^2)$ iterations. 
}
\begin{proof}


Recall, the task is to find a $k$ such that the interval identified by~\ref{step:interval} is less than $\frac{1}{\mathsf{bound}_{\mathsf{diff}}}$.
Note that $\mathsf{bound}_{{\opt}} < \mathsf{bound}_{\mathsf{diff}}$. Therefore, $\frac{1}{\mathsf{bound_{diff}}} < \frac{1}{\mathsf{bound_{v}}}$. Hence, there can be only one rational value with denominator $\mathsf{bound}_{\mathsf{\opt}}$ or less in the small interval identified by the chosen $k$. Since the optimal value must also lie in this interval, the unique rational number with denominator $\mathsf{bound}_{\mathsf{\opt}}$ or less must be the optimal value. 
Let $k$ be such that the interval from~\ref{step:interval} is less than $\frac{1}{\mathsf{bound}_{\mathsf{diff}}}$.
Then, 
\begin{align*}
     2\cdot\frac{\mu}{d-1\cdot d^{k-1}} \leq &  c\cdot \frac{1}{(p^{(|V|^2)} - q^{(|V|^2)})\cdot (p^{(|V|^2)})} \text{ for some  } c>0  \\
    2\cdot\frac{\mu}{d-1\cdot d^{k-1}} \leq & c\cdot \frac{q^{2\cdot |V|^2}}{(p^{(|V|^2)} - q^{(|V|^2)})\cdot (p^{(|V|^2)})} \text{ for some  } c>0  \\
    2\cdot\frac{\mu}{d-1\cdot d^{k-1}} 
     \leq & 
     c\cdot \frac{1}{(d^{(|V|^2)} - 1)\cdot (d^{(|V|^2)})} \text{ for  } c>0  \\
    d-1\cdot d^{k-1} \geq &
     c' \cdot \mu \cdot (d^{(|V|^2)} - 1)\cdot (d^{(|V|^2)}) \text{ for   } c'>0 \\
     2\cdot\log(d-1) + k\cdot \log(d) \geq &
     c'' + \log(\mu) + \log(d^{(|V|^2)} - 1) +  {|V|^2}\cdot\log(d) \text{ for   } c''>0 
\end{align*}

The following cases occur depending how large or small the values are:

\begin{enumerate} [label= Case \arabic*.]
    \item When $d\geq 2$:  
    In this case, both $d$ and $d^{|V|^2}$ are large. Then, 
    \begin{align*}
        2\cdot\log(d-1) + k\cdot \log(d) & \geq 
     c'' + \log(\mu) + \log(d^{(|V|^2)} - 1) +  {|V|^2}\cdot\log(d) \text{ for  } c''>0 \\
     2\cdot\log(d) + k\cdot \log(d) & \geq 
     c'' + \log(\mu) + {(|V|^2)}\log(d) +  {|V|^2}\cdot\log(d) \text{ for  } c''>0 \\
     k & = \O(|V|^2)
    \end{align*}
    
    
    \item When $d$ is small but $d^{|V|^2}$ is not: In this case, $\log(d) \approx (d-1)$, and $\log(d-1) \approx 2-d$. Then,
     \begin{align*}
        2\cdot\log(d-1) + k\cdot \log(d) & \geq 
     c'' + \log(\mu) + \log(d^{(|V|^2)} - 1) +  {|V|^2}\cdot\log(d) \text{ for  } c''>0 \\
     2\cdot\log(d-1) + k\cdot \log(d) & \geq 
     c'' + \log(\mu) + {(|V|^2)}\log(d) +  {|V|^2}\cdot\log(d) \text{ for  } c''>0 \\
     2\cdot (2-d) + k\cdot (d-1) & \geq 
     c'' + \log(\mu) + {(|V|^2)}(d-1) +  {|V|^2}\cdot (d-1) \text{ for  } c''>0 \\
     k = \O\Big(\frac{\log(\mu)}{d-1} + |V|^2\Big)
    \end{align*}
    
    
    \item When both $d$ and $d^{|V|^2}$ are small. Then, in addition to the approximations from the earlier case, $ \log(d^{|V|}-1) \approx (2-d^{|V|})$. So, 
     \begin{align*}
        2\cdot\log(d-1) + k\cdot \log(d) & \geq 
     c'' + \log(\mu) + \log(d^{(|V|^2)} - 1) +  {|V|^2}\cdot\log(d) \text{ for  } c''>0 \\
     2\cdot\log(d-1) + k\cdot \log(d) & \geq 
     c'' + \log(\mu) + 2-d^{(|V|^2)} +  {|V|^2}\cdot\log(d) \text{ for  } c''>0 \\
     2\cdot (2-d) + k\cdot (d-1) & \geq 
     c'' + \log(\mu) + 2-d^{(|V|^2)} +  {|V|^2}\cdot (d-1) \text{ for  } c''>0 \\
     k = \O\Big(\frac{\log(\mu)}{d-1} + |V|^2\Big)
    \end{align*}
    
\end{enumerate}

\qed 
\end{proof}



\subsubsection{Concrete example to establish $\Omega(|V|)^2$ lower bound for number of iterations required by the value iteration algorithm}
\\
Recall Fig~\ref{fig:lowerboundexample}, as presented here as well:
\begin{figure}[h]
\vspace{0cm}
    \centering
    
    \begin{tikzpicture}[shorten >=1pt,on grid,auto] 
   
    \node[state] (q_1) {\footnotesize{Start}};
    \node[state] (q_2)  [right of = q_1, node distance=2cm, minimum size=0.5cm] {};
    \node[state] (q_3)  [left of = q_1, node distance=2cm, minimum size=0.5cm] {};
    \node[] (q_4)  [right of = q_1, node distance=5cm] {\Large{\textellipsis}};
    \node[] (q_5) [left of=q_3, node distance=1.8cm]
    {\Large\textellipsis};
    \node[state] (q_6) [below right of = q_2, minimum size=0.5cm, node distance=1cm];
    \node[state] (q_7) [above left of = q_3, minimum size=0.5cm, node distance=1cm];
  
    \path[->] 
    (q_1) edge  node {$w>0$} (q_2)
          edge  node [above] {$0$} (q_3)
         
    (q_2) edge [bend right = 20] node {1} (q_6) 
    (q_6) edge [bend right = 40, dashed] node   {0} (q_4) 
    (q_3) edge [bend right = 20] node {1} (q_7) 
    (q_7) edge [bend right = 40, dashed] node   {0} (q_5) 
    (q_4) edge [bend right = 80, dashed] node  {0} (q_2)
    (q_5) edge [bend right = 80, dashed] node {0} (q_3);
    \end{tikzpicture}
    \caption{Sketch of game graph which requires $\Omega(|V|^2)$ iterations}
%\end{wrapfigure} 
\end{figure}

Let the left hand side loop have $4n$ edges, the right hand side of the loop have $2n$ edges, and $w = \frac{1}{d^{3n}} + \frac{1}{d^{7n}} + \cdots + \frac{1}{d^{m\cdot n -1}}$ such that $m\cdot n -1 = c\dcot n^2$
for a positive integer $c>0$.


One can show for a finite games of length  $(m\cdot n -1)$ or less, the optimal path arises from the loop to the right. But for games of length greater than  $(m\cdot n -1)$, the optimal path will be to due to the left hand side loop. 



\subsubsection{Theorem~\ref{Thrm:DSFull}}
{\em 
%[Safety and co-safety properties of DS-comparators]
Let $\mu>1$ be the upper bound.  
For arbitrary discount factor $d>1$ and threshold value $v$
\begin{enumerate}
\item {\label{Item:Safety}}  DS-comparison languages are safety languages for relations $R \in \{\leq, \geq, =\}$.
%non-strict inequalities and the equality relation
\item {\label{Item:CoSafety}} DS-comparison language are co-safety languages for relations $R \in \{<, >, \neq\}$.
\end{enumerate}
}
\begin{proof}
Due to duality of safety/co-safety languages, it is sufficient to show that DS-comparison language with $ \leq$ is a safety language. 


Let us assume that DS-comparison language with $ \leq$  is not a safety language. Let $W$ be a weight-sequence in the complement of DS-comparison language with $ \leq$  such that it does not have a bad prefix. 

Since $W $ is in the complement of DS-comparison language with $ \leq$, $\DSum{W}{d} > v$. By assumption, every $i$-length prefix $W[i]$ of $W$ can be extended to a bounded weight-sequence $W[i]\cdot Y^i$ such that $\DSum{W[i]\cdot Y^i}{d} \leq v$. 

\sloppy
Note that  $\DSum{W}{d} = \DSum{\pre{W}{i}}{d} + \frac{1}{d^i} \cdot \DSum{\suf{W}{i}}{d}$, and $\DSum{\pre{W}{i}\cdot Y^i}{d} = \DSum{\pre{W}{i}}{d} + \frac{1}{d^i} \cdot \DSum{Y^i}{d}$. The contribution of tail sequences $\suf{W}{i}$ and $Y^i$ to the discounted-sum of $W$ and $\pre{W}{i}\cdot Y^i$, respectively diminishes exponentially as the value of $i$ increases. In addition, since and $W$ and  $\pre{W}{i}\cdot Y^i$ share a common $i$-length prefix $\pre{W}{i}$, their discounted-sum values must converge to each other.
The discounted sum of $W$ is fixed and greater than $v$, due to convergence there must be a $k\geq  0$ such that $\DSum{\pre{W}{k}\cdot Y^k}{d} > v$. Contradiction. 
Therefore, DS-comparison language with $ \leq$  is a safety language. 

The above intuition is formalized below:

Since $\DSum{W}{d} > v$ and $\DSum{\pre{W}{i}\cdot Y^i}{d} \leq v$, the difference $\DSum{W}{d} - \DSum{\pre{W}{i}\cdot Y^i}{d} > 0$. 

By expansion of each term, we get $\DSum{W}{d}- \DSum{\pre{W}{i}\cdot Y^i}{d} = \frac{1}{d^i}(\DSum{\suf{W}{i}}{d} - \DSum{Y^i}{d}) \leq  \frac{1}{d^i}\cdot(\mod{\DSum{\suf{W}{i}}{d}}  + \mod{\DSum{Y^i}{d}} )$. Since the maximum value of discounted-sum of sequences bounded by $\mu$ is $\frac{\mu\cdot d}{d-1}$, we also get that $\DSum{W}{d}- \DSum{\pre{W}{i}\cdot Y^i}{d} \leq 2\cdot \frac{1}{d^{i}} \mod{ \frac{\mu\cdot d}{d-1}} $. 

Putting it all together, for all $i\geq 0$ we get
\[
0< \DSum{W}{d} - \DSum{W[i]\cdot Y^i}{d} \leq 2\cdot \frac{1}{d^{i}} \mod{\frac{\mu\cdot d}{d-1}} 
\]
As $i \rightarrow \infty$, $2\cdot \mod{\frac{1}{d^{i-1}}\cdot \frac{\mu}{d-1}} \rightarrow 0$. So, $\lim_{i \rightarrow \infty} (\DSum{W}{d} - \DSum{W[i]\cdot Y^i}{d}) = 0$. Since $\DSum{W}{d}$ is fixed, $\lim_{i \rightarrow \infty}\DSum{W[i]\cdot Y^i}{d} = \DSum{W}{d}$.
%Therefore, $\lim_{i \rightarrow \infty}\DSum{W[i]\cdot Y^i}{d} > 0 $.

By definition of convergence, there exists an index $k\geq 0$ such that $\DSum{W[k]\cdot Y^k}{d}$ falls within the  $\frac{\mod{\DSum{W}{d}}}{2}$ neighborhood of $\DSum{W}{d}$. Finally since $\DSum{W}{d}> 0$, $\DSum{W[k]\cdot Y^k}{d} > 0$ as well. But this contradicts our assumption that for all $i \geq 0$, $\DSum{W[i]\cdot Y^i}{d} \leq 0$.

Therefore, DS-comparator with $ \leq$  is a safety comparator. 
\qed 
\end{proof}

\subsubsection{Lemma~\ref{Lem:GapThreshold}}
{\em 
	Let $\mu>0$ be the integer upper bound,  $d >1$ be an integer discount factor, and the relation $\R$ be the inequality $\leq$. 
	Let $v \in \Q$ be the threshold value such that 
	 $v = v[0]v[1]\dots v[m](v[m+1]v[m+2]\dots v[n])^{\omega}$.
	Let $W$ be a non-empty, bounded, finite weight-sequence.   
	Then, weight sequence $W$ is a bad-prefix of the DS comparison language with $\mu$, $d$, $\leq$ and $v$ iff $\gap{W-\pre{v}{|W|}} >  \frac{1}{d}\cdot \DSum{\post{v}{|W|}}{d} + \frac{\mu}{d-1}$.
}
\begin{proof}
\sloppy
Let $W$ be a bad prefix. Then for all infinite length, bounded weight sequence $Y$ we get that $\DSum{W\cdot Y}{d} > v \implies \DSum{W}{d} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d} \geq \DSum{\pre{v}{|W|}\cdot\post{v}{|W|}}{d} \implies \DSum{W}{d} - \DSum{\pre{v}{|W|}}{d} > \frac{1}{d^{|W|}}\cdot (\DSum{\post{v}{|W|}}{d} - \DSum{Y}{d})\implies \gap{W-\pre{v}{|W|}} > \frac{1}{d} (\DSum{\post{v}{|W|}}{d} + \frac{\mu\cdot d}{d-1})$.

Next, we prove that if a finite weight sequence $W$ is such that, the W is  a bad prefix. Let $Y$ be an arbitrary infinite but bounded weight sequence. Then $\DSum{W\cdot Y}{d} 
= \DSum{W}{d} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d} 
= \frac{1}{d^{|W|-1}}\cdot \gap{W} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d} 
= \frac{1}{d^{|W|-1}}\cdot \gap{W} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d} + \frac{1}{d^{|W|-1}}\cdot (\gap{\pre{v}{|W|}} - \gap{\pre{v}{|W|}})
$. By re-arrangement of terms we get that 
$\DSum{W\cdot Y}{d}
= \frac{1}{d^{|W|-1}}\cdot \gap{W-\pre{v}{|W|}} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d} + \frac{1}{d^{|W|-1}}\cdot \gap{\pre{v}{|W|}}$. Since 
 $ \gap{W - \pre{v}{|W|}} > \frac{1}{d}\cdot (\DSum{\post{v}{|W|}}{d} + \frac{\mu\cdot d}{d-1})$ holds, we get that 
 $\DSum{W\cdot Y}{d} 
 >  \frac{1}{d^{|W|}}\cdot (\DSum{\post{v}{|W|}}{d} + \frac{\mu\cdot d}{d-1}) +  \frac{1}{d^{|W|}}\cdot \DSum{Y}{d} + \frac{1}{d^{|W|-1}}\cdot \gap{\pre{v}{|W|}}$. Since minimal value of $\DSum{Y}{d} is \frac{-\mu\cdot d}{d-1}$, the inequality simplifies to  $\DSum{W\cdot Y}{d} > \frac{1}{d^{|W|-1}}\cdot \gap{\pre{v}{|W|}} + \frac{1}{d^{|W|}}\cdot \DSum{\post{v}{|W|}}{d}  \implies \DSum{W\cdot Y}{d} > \DSum{v}{d} = v$. Therefore, $W$ is a bad prefix. 
\qed
\end{proof}


\subsubsection{Lemma~\ref{Lem:GapThresholdVeryGood}}
{\em 
Let $\mu$ and $d>1 $ be the bound and discount-factor, resp.
Let $W$ be a non-empty, bounded, finite weight-sequence.   
Weight sequence $W$ is a very good-prefix of $\A^{\mu,d}_\leq$ iff $\gap{W-\pre{v}{|W|}} \leq \frac{1}{d}\cdot \DSum{\post{v}{|W|}}{d} - \frac{\mu}{d-1}$.
	}

\begin{proof}
Let $W$ be a very good prefix. Then for all infinite, bounded sequences $Y$, we get that $\DSum{W\cdot Y}{d} \leq v \implies \DSum{W}{d} + \frac{1}{d^{|W|}} \cdot \DSum{Y}{d} \leq v$. By re-arrangement of terms, we get that $\gap{W-\pre{v}{|W|}} \leq \frac{1}{d}\cdot \DSum{\post{v}{|W|}}{d} - \frac{1}{d}\cdot \DSum{Y}{d}$. Since maximal value of $\DSum{Y}{d} = \frac{\mu\cdot d}{d-1}$, we get that $\gap{W-\pre{v}{|W|}} \leq \frac{1}{d}\cdot \DSum{\post{v}{|W|}}{d} - \frac{\mu}{d-1}$.

Next, we prove the converse. We know 
$\DSum{W\cdot Y}{d} 
= \DSum{W}{d} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d}
= \frac{1}{d^{|W|-1}}\cdot \gap{W} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d}
= \frac{1}{d^{|W|-1}}\cdot \gap{W} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d} +   \frac{1}{d^{|W|-1}}\cdot (\gap{\pre{v}{|W|}} - \gap{\pre{v}{|W|}})
$. 
By re-arrangement of terms we get that 

\sloppy
$\DSum{W\cdot Y}{d}
=\frac{1}{d^{|W|-1}}\cdot \gap{W-\pre{v}{|W|}} + \frac{1}{d^{|W|}}\cdot \DSum{Y}{d} + \frac{1}{d^{|W|-1}}\cdot\gap{\pre{v}{|W|}}$. From assumption we derive that 
$\DSum{W\cdot Y}{d} \leq \frac{1}{d^{|W|}}\cdot \DSum{\post{v}{|W|}}{d} - \frac{\mu}{d-1} + \frac{1}{d^{|W|}}\cdot\DSum{Y}{d}  + \DSum{\pre{v}{|W|}}{d}$. Since maximal value of $\DSum{Y}{d}$ is $ \frac{\mu}{d-1}$, we get that $\DSum{W\cdot Y}{d}\leq v$. Therefore, $W$ is a very good prefix.
\qed
\end{proof}


\subsubsection{Lemma~\ref{lem:one-one-plays}}
{\em 
There is a one-one correspondence between plays in $G$ and plays in $\GA$. This correspondence preserves the winning condition. 
}
\begin{proof}

(One-one correspondence) 
Let $\rho = v_0v_1\dots$ be a play in $G$ with cost sequence $w_0w_1\dots$. 
Let $s_0s_1\dots$ be the run of weight cost  of $w_0w_1\dots$ in the DS comparator. Note, that since the comparator is deterministic, there is a unique run for each finite/infinite cost sequence. 
Then, play $\rho  = v_1v_2\dots$ in $G$ and corresponds to play $(v_0,s_0)(v_1,s_1)\dots$ in $\GA$.
Similarly, one can prove that for each play $(v_0,s_0)(v_1,s_1)\dots$ in $\GA$ uniquely corresponds to play $v_0v_1\dots$ in $G$, where the correspondence is defined by the weight sequence shared by the run $s_0s_1\dots$ in the comparator and play $v_0v_1\dots$ in $G$.

(Winning-condition preservation) 
A play $\rho = v_0v_1v_2\dots$ is a winning run for player $P_1$ in $G$ iff its cost relates to threshold value $v$ by $\R$. So, let $n_1n_2\dots$ be the cost sequence of $\rho$ in G, then $\DSum{n_1n_2\dots}{d}$ $\R$ $v$ holds. 
Let the run of weight sequence $n_0n_1\dots$ be $s_0s_1s_2\dots$ in comparator automata $ \A$. Then, run $s_0s_1s_2\dots $ is an accepting run in $\A$. As a result, the corresponding play in $\GA$, i.e. $s_0s_1s_2\dots$ must be a winning run in $G$.
\end{proof}

==> Chapters/integergames/Section/nonintegerDF.tex <==
\section{For non-integer discount factors}

\input{Section/lowerapproximation.tex}

\input{Section/lowerapproxcomparator.tex}





==> Chapters/integergames/Section/prelims.tex <==
\section{Preliminaries}
\label{Sec:Prelims}
%The preliminaries are split into game-theoretic and language-theoretic concepts.


==> Chapters/integergames/Section/problemstatement.tex <==

\section{Problem statement}

Typically, one solves the optimization problem on quantitative games which is to determine the best costs that each player can procure, assuming that the objectives of player $P_0$ and $P_1$ oppose each other in terms of maximizing and minimizing the costs. 
The optimal cost may not only not be required but also not computed precisely due to optimization based algorithms.
Instead, we solve the {\em satisficing problem} where the goal is to determine whether a player can guarantee that the cost remains within a given threshold. As  a result, the satisficing problem is a decision problem, stated as follows:

\subsection*{Decision problem}

%As earlier, the objectives of player $P_0$ and $P_1$ are to maximize and minimize their costs from the game. 

In the decision problem the question is whether $P_1$ has a strategy such that it is guaranteed to never exceed a cost threshold. In this case, we assume adversarial behavior from player $P_0$, and refer to it as the {\em opponent}.
%that its cost never exceeds a fixed amount. 


Formally, given a cost-threshold $v \in \R$, player $P_1$ is said to have a {\em winning strategy with cost-threshold $v$} if there exists a strategy $V^*V_1 \rightarrow V$ such that for all strategies of the opponent, the cost of the resulting play does not exceed a cost of $v$. The decision problem asks whether  given a cost-threshold $v \in \R$ player $P_1$ has a winning strategy with threshold $v$. 

The satisficing problem can be solved using the optimization problem, in this work we show that solving the satisficing problem alone has advantages of its own.  

\subsection{Objective}
The optimization problem solves the decision problem as well. If the optimal value $W$ is less than or equal to cost threshold  $v \in R$, then player $P_1$ will have a winning strategy with threshold $v$, otherwise it won't. This procedure is $\O(|V|^2)$ or $\O(|V|^4)$ depending on how large the maximum cost on transitions in the game graph is. 
In this document, we show that when the discount factor is an integer, the decision problem can be solved more efficiently via a reduction to  reachability/safety games.

\begin{comment}

\subsubsection{Our approach}
\begin{center}
    Comparator-based symbolic approach! 
\end{center}
\begin{enumerate}
    \item Construct comparator automata with discount factor $d>1$ and value $v$ that accepts an infinite bounded sequence $W$ iff $\DSum{W}{d}$ $R$ $v$, where $R \in \{\leq, <, =, >, \geq\}$.
    
    \item If comparator automata is $\omega$-regular, take product of quantitative graph game and comparator to obtain a graph game with winning states. 
    
    \item Prove that $\omega$-regular comparator automata is safety/co-safety automata, therefore resulting graph game is safety/co-safety graph games. Therefore, solving this game is easier. 
\end{enumerate}

\subsubsection{Results proven so far}
\begin{enumerate}
    \item (Theorem~\ref{Thrm:DSFull}) Define the discounted-sum comparison language with discount factor $d>1 $, threshold $v\in \Re$, relation $\R$ and upper bound $\mu>0$ to be the language that accepts infintie bounded weight sequences $W$ iff $\DSum{W}{d}$ $\R$ $v$ holds. 
    \begin{enumerate}
        \item We prove that DS comparison language is a safety language for all $d>1$, $v$ and $\mu$ if $\R \in \{\leq, \geq, =\}$
        
        \item   We prove that DS comparison language is a co-safety language for all $d>1$, $v$ and $\mu$ if $\R \in \{<, >, \neq\}$
    \end{enumerate}
  
    \item Let threshold value $v$  be represented by the regular expression $v[0]v[1]\dots v[m](v[m+1]v[m+2]\dots v[n])^{\omega}$ such that $v = \DSum{v[0]v[1]\dots}{d}$. By abuse of notation, we denote all three- the regular expression $ v[0]v[1]\dots v[m](v[m+1]v[m+2]\dots v[n])^{\omega}$, the value of $\DSum{v}{d}$ and the real number $v$ - by $v$. The notation will be clear in context, and clarified otherwise. 
    
    (Theorem~\ref{thrm:regularWithVal})
    Let $d>1$ be an integer discount factor. Let $v\in\Re$ be represented as above. Then the DS comparator automata for integer discount factor $d>1$, threshold $v$, relation $\R$ and upper bound $\mu>0$ is $\omega$-regular.
    
    \item (Corollary~\ref{coro:regularWithVal})
    We provide  deterministic safety and co-safety automata constructions for the DS comparators defined above. 
    
    For integer discount factor $d>1$, threshold value $v = v[0]v[1]\dots v[m](v[m+1]v[m+2]\dots v[n])^{\omega}$, and upper bound $\mu>0$, the number of states in the deterministic safety/co-safety automata is $\O(\frac{\mu\cdot n}{d-1})$.
    
    \item (Theorem~\ref{thrm:reduction}) Quantitative game synthesis is reduced to game solving of a safety/co-safety graph game, depending on $\R$, with $\O(|V|\cdot\frac{\mu\cdot n}{d-1})$ states.  
    
\end{enumerate}

\end{comment}

\begin{comment} 
\subsubsection{Possible TODOs}
\begin{enumerate}
    \item What is symbolic representation of quantitative graph games? Maybe, BDD/SAT-based symbolic encoding and  implementation? Use $\mathsf{SSyft}$?
    \item Application?
    \begin{itemize}
        \item Combine qualitative specifications with quantitative ones. Attempt to demonstrate that overhead of quantitative constraint is low.
        \item Find a concrete application within Robotics?
    \end{itemize}
    \item Extension to non-integer discount factors.
    \begin{itemize}
        \item What is the corresponding anytime/approximation synthesis scheme?
    \end{itemize}
\end{enumerate}

\end{comment}

==> Chapters/integergames/abstract.tex <==

\begin{abstract}
Several problems in planning and reactive synthesis are reduced to the analysis of two-player quantitative graph games. 
{\em Optimization} is one form of analysis.
We argue that in many cases the optimization problem can be replaced by a {\em satisficing problem}, wherein instead of determining the optimal value to win the game, the problem determines whether the game can be won within a given threshold bound. 

This work defines and investigates the satisficing problem on a two-player graph game where the cost model is given by the discounted-sum aggregate function. 
When the discount factor is an integer, we present  a purely automata-based solution to the problem that uses {\em comparator automata}, and show that satisficing can be solved in linear time of the size of the game. 
We also observe that traditional solutions for optimization, which are based on numerical methods, can be adapted to solve satisficing.  But numerical solutions for both problems, optimization and satisficing, exhibit 
polynomial-time solutions of degrees that are too large to be scalable.
An empirical evaluation not only supports the aforementioned theoretical observations but reveals further practical advantages of automata-based methods over numerical methods. 
\end{abstract}


==> Chapters/integergames/macro.tex <==
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage{amsfonts}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{graphicx}
%\usepackage{hyperref}
\usepackage[bookmarks=false]{hyperref}
\usepackage{listings}
\usepackage{makeidx}  % allows for indexgeneration
%\usepackage{smallsec} % self-style file
%\usepackage[compact]{titlesec}
\usepackage{subcaption}
\usepackage{url}
\usepackage{wrapfig}

%tikz package 
\usepackage[graphicx]{realboxes}
\usepackage{tikz}
\tikzset{elliptic state/.style={draw,ellipse}}
\usetikzlibrary{shapes,shapes.geometric,arrows,fit,calc,positioning,automata,}
\usetikzlibrary{automata,positioning}
\usepackage{tikz-qtree}
\usepackage{float}
\usepackage{floatflt}

%BAD PREFIXES 
\newcommand{\bad}{bad}
\newcommand{\verygood}{very-good}

%General macros
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\Z}{\mathbb{Z}}
\renewcommand*{\L}{\mathcal{L}}
\renewcommand*{\O}{\mathcal{O}}
\newcommand{\ol}[1]{\overline{#1}}
\renewcommand*{\Re}{\mathbb{R}}
\newcommand*{\cct}[1]{\textsf{#1}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\GA}{\mathsf{GA}}


%General math macros
\renewcommand*{\mod}[1]{|#1|}
\newcommand*{\ceil}[1]{\lceil #1 \rceil}
\newcommand*{\floor}[1]{\lfloor #1 \rfloor}

%General automata-theroetic notations
\newcommand*{\A}{\mathcal{A}}
\newcommand*{\Statess}{\mathit{S}}
\newcommand*{\State}{S}
\newcommand*{\Start}{s_I}
\newcommand*{\Final}{\mathcal{F}}
\newcommand*{\StartState}{{\mathit{Init}}}
\newcommand*{\AcceptingStates}{S_{acc}}
\newcommand*{\wt}{\mathit{wt}}
\newcommand*{\sink}{\mathsf{sink}}
\newcommand*{\init}{v_\mathit{init}}


%Safety macros
\newcommand*{\pre}[2]{#1[\cdots#2]}
\newcommand*{\post}[2]{#1[#2\cdots]}
\newcommand*{\suf}[2]{#1[#2\dots]}
\newcommand{\gap}[1]{\mathsf{gap}(#1,d)}
\newcommand{\thresh}{\mathsf{T}}

%macros for DS
\newcommand*{\DSum}[2]{\mathit{DS}({#1}, {#2})}
\newcommand*{\MaxC}{\mathit{maxC}}
\newcommand*{\MaxX}{\mathit{maxX}}
\newcommand*{\R}{\mathsf{R}}
\newcommand*{\transwt}{\mathsf{cost}}
\newcommand*{\opt}{W}

%macos for round and gap
%\newcommand{\roundL}[1]{\mathsf{roundLow}(#1,k,p)}
%\newcommand{\roundU}[1]{\mathsf{roundUpper}(#1,k,p)}
%\newcommand{\gapL}[1]{\mathsf{gapLower}(#1,k,p)}
%\newcommand{\gapU}[1]{\mathsf{gapUpper}(#1,k,p)}
%\newcommand{\DSumL}[1]{\mathsf{DSLow}(#1,k,p)}
%\newcommand{\DSumU}[1]{\mathsf{DSUpper}(#1,k,p)}

\newcommand{\todo}[1]{\textbf{TODO}{#1}}

%macros for tools
\newcommand{\optimize}{\mathsf{VIOptimal}}
\newcommand{\compSatisfice}{\mathsf{CompSatisfice}}
\newcommand{\visatisfice}{\mathsf{VISatisfice}}
%marcros for math env. 
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{definition}{Definition}
